Active Sampling for Accelerated MRI with Low-Rank Tensors

Magnetic resonance imaging (MRI) is a powerful imaging modality that revolutionizes medicine and biology. The imaging speed of high-dimensional MRI is often limited, which constrains its practical utility. Recently, low-rank tensor models have been exploited to enable fast MR imaging with sparse sampling. Most existing methods use some pre-defined sampling design, and active sensing has not been explored for low-rank tensor imaging. In this paper, we introduce an active low-rank tensor model for fast MR imaging. We propose an active sampling method based on a Query-by-Committee model, making use of the benefits of low-rank tensor structure. Numerical experiments on a 3-D MRI data set demonstrate the effectiveness of the proposed method.

==> ICIP'21_Active_tensor_MRI/active_strategy.tex <==
\section{Active Tensor Sampling Method}
\label{sec:active_strategy}
The complete flowchart of our MRI reconstruction framework is illustrated in Fig.~\ref{fig:whole_framework}. In order to design an active sampling method for MRI reconstruction, two questions need to be answered: (1) How can we pick informative samples? (2) How can we guarantee that the new samples obey the patterns of MRI scans? We will provide the details in this section.


\subsection{Query-by-Committee-based Active Sampling}
\label{sec:element_sample}
We are inspired by a classical active learning approach called Query-by-Committee~\cite{seung1992query}. The key idea is to employ a committee of different models to predict the values at some candidate samples respectively. With such a committee, we can measure the quality of a candidate sample and pick the optimal one. The two key components of the Query-by-Committee approach are
\begin{itemize}[leftmargin=*]
    \item{\bf A committee of models.} The different mode-unfolding matrices obtained from solving Eq.~\reff{eq:raw_Obj} naturally form a committee required by our active sampling. 
    This model committee enables us to define an element-wise utility measure, denoted as $u(\xi)$, where $\xi$ is an element in the tensor. 
    \item {\bf Measure of sample quality.} After constructing a committee of models, we can define a measure of sample quality $u$. The sample with the maximized $u$ will be selected and added into the observation set: $\Omega \leftarrow \Omega \cup \argmax_{\xi}~u\left( {\xi} \right)$. We consider the predictive variance and leverage score as well as their combinations as our measure of sample quality, as detailed in the next sub-section.
\end{itemize} 

\subsection{Measure of Sample Quality}
{\bf Predictive variance.} The first choice is the predicted variance from different tensor modes. Based on the solved ${\mat{X}_n}$, if we unfold it and 
    enforcing its consistency with the observed data, we can obtain mode-$i$ low-rank approximation to $\ten{M}$:  
    %, inspired from the classical measure, namely the disagreement among models.
    %From the Sub-${\mat{X}_i}$ problems of our previous alternating algorithms, we can obtain a low-rank approximation tensor for one specific mode of the reconstructed tensor $\ten{M}$ via folding ${\mat{X}_i}$. 
    %Each one is a low-rank approximation for one specific mode of the reconstructed tensor $\ten{M}$. 
    %Therefore, after enforcing the consistency with the observed data, ${\tilde{\ten{M}}_i}$ can be seen as a mode-$i$ approximation to $\ten{M}$:
\begin{equation} 
\label{eq:mode_appro}
\begin{aligned}
& {\tilde{\ten{M}}_n} {\rm{ := }}  {{{\text{Fold}_n}(\mat{X}}_n}), \quad {\tilde{\ten{M}}_n}(\Omega) \leftarrow  \ten{T}(\Omega).
\end{aligned}
\end{equation}
Let $\mathbb{E}\left[ {\tilde{\ten{M}}} \right] := \sum_{n = 1}^N {{w_n}{{\tilde{\ten{M}}}_n}}$ be the reconstructed tensor,
%the weighted average tensor of $n$ mode approximations, 
we define the difference tensor of each approximation ${\Delta \ten{M}_n}$ and the predictive variance tensor $\ten{V}$ as:
% \begin{equation}
% \label{eq:diff_measure}
% {\Delta \ten{M}_n} := {\tilde{\ten{M}}_i} - \mathbb{E}\left[ {\tilde{\ten{M}}} \right] 
% \end{equation}
\begin{equation}
\label{eq:var_measure}
{\Delta \ten{M}_n} := {\tilde{\ten{M}}_n} - \mathbb{E}\left[ {\tilde{\ten{M}}} \right],\; \; \ten{V} := \sum\limits_{n = 1}^N {{w_n}} {\left( {\Delta \ten{M}_n} \circ {\Delta \ten{M}_n} \right)}
\end{equation}
% with
% \begin{equation}
% {w_i} = \begin{cases} 
% {{\lambda_i}} / {\sum\nolimits_i {{\lambda_i}} } & \text{if block-coordinate descent is used}\\
% 1 / n &  \text{if ADMM is used},
% \end{cases}   
% \end{equation}
%Complex version ??
where $\circ$ denotes a Hadamard product, and ${w_n}$ is the weight associated with mode-$n$ approximation ${{\tilde{\ten{M}}}_n}$. The value of ${w_n}$ depends on the solver to Eq.~\reff{eq:raw_Obj}. In our implementation, we adopt an ADMM solver and have $\{w_n\}_{n=1}^N = \tfrac{1}{N}$.
% \begin{equation}
% \mathbb{E}\left[ {\tilde{\ten{M}}} \right] := \sum\limits_{i = 1}^n {{w_i}{{\tilde{\ten{M}}}_i}}.     
% \end{equation}

Note that the predicted variance is a semi-variance that is defined to measure the disagreement among different modes. Since the consistency of the observed data is enforced, the committee has zero disagreement on them. Maximizing the predictive variance helps to identify the sample with large prediction error.
%Among the $n$ mode approximation tensors $\left\{{\tilde{\ten{M}}_i}\right\}_{i=1}^n$, some of the estimated entries are the same or similar with the true data (with small variance), while some other estimated entries are very different (with large variance). 
%Therefore, we can treat $\ten{V}$ as a measure of disagreement. 
The following lemma describes the relation between the reconstructed error and the predictive variance.
\begin{lemma}
Let ${\mu}$ be the sum of all elements of the predictive variance tensor
$\mu:= \|{\rm vec}(\ten{V}) \|_1 = \sum\limits_{n = 1}^N {{w_n}} {\left\| {\Delta \ten{M}_n} \right\|_{\rm F}^2}$, ${\mu_i}$ be the mode-$n$ approximation error: ${\mu_n}=\left\|\ten{M} - {\tilde{\ten{M}_n}} \right\|_{\rm F}^2$, and ${\mu _{\rm rec}}$ be the reconstruction error of the whole data set: $\mu _{\rm rec}=\left\|\ten{M}-\mathbb{E}\left[ {\tilde{\ten{M}}} \right] \right\|_{\rm F}^2$, we have
\begin{equation}
\label{eq:relation_err_var}
{\mu _{\rm rec}} = \sum\limits_{n = 1}^N {w_n}{\mu_n } - \mu.
\end{equation}
\end{lemma}
\begin{comment}
\begin{proof}
Given two tensors $\ten{A}$ and $\ten{B}$ which are of the same size, we have $\|\ten{A} - \ten{B}\|_{\rm F}^2 = \|\ten{A}\|_{\rm F}^2 + \|\ten{B}\|_{\rm F}^2 - 2 \| {\rm {vec}}(\ten{A} \circ \ten{B})\|_1$. Eq.~\eqref{eq:relation_err_var} is obtained by applying such an expansion on $\mu$, $\mu_i$ and $\mu _{\rm rec}$.
\end{proof}
\end{comment}
The approximations of different modes gradually converge to the same one as more samples are observed. 
%When the tensor is fully sampled, both $\mu$ and $\mu_{\rm rec}$ approach zero.
A sample with the maximized predictive variance help to $\mu_{\rm rec}$ decreases quickly. The similar idea is used to reduce generalization error in the ensemble  learning~\cite{mendes2012ensemble}.


{\bf Leverage score.} Our second quality measurement $u$ is the leverage score. It comes from the incoherence property of a matrix~\cite{candes2009exact}.
%: a low-rank matrix can be recovered via nuclear norm minimization if it satisfies the incoherent property.
%, which means that the theory xxx (matrixsampling2017.pdf)
Given the singular value decomposition (SVD) of a rank-$R$ matrix $\mat{A}= \mat{U}\mat{\Sigma} {\mat{V}^H} \in {\mathbb{C}^{{N_1}\times{N_2}}}$, let $\mat{e}_i$ be the $i$-th standard basis, 
%\hzc{Check the generalization in complex number}
the left and right leverage scores of a matrix are defined as:
\begin{equation}
\begin{array}{l}
{\boldsymbol{\ell}(i)} := \frac{N_1}{R}{\left\| {{\mat{U}^T}{\mat{e}_i}} \right\|^2_2},\quad i = 1,2,\ldots,{N_1}, \\
{\mat{r}(j)} := \frac{N_2}{R}{\left\| {{\mat{V}^T}{\mat{e}_j}} \right\|^2_2},\quad j = 1,2,\ldots,{N_2}.
\end{array}
\end{equation}
%The leverage scores can be also estimated from a partially observed matrix~\cite{eftekhari2018mc2}. 
A leverage score measures the coherence of a row/column with a coordinate direction, which generally reflect the importance of the rows/columns.
%Generally, the rows/columns with larger left/right scores are more informative.
For the mode-$n$ approximation $\mat{X}_n$, we can perform SVD and calculate its left and right leverage scores as $\boldsymbol{\ell}_n$ and $\mat{r}_n$ respectively, then the element-level leverage score of a sample $\left(i,j \right)$ in $\mat{X}_n$ is defined as:
\begin{equation}
\label{eq:mode_lev_measure}
{{l_n} \left(i,j\right)}: = {\boldsymbol{\ell}_n(i)} \cdot {\mat{r}_n(j)},\quad n=1,2,\ldots,N.
\end{equation}
%It is reasonable to assume that the samples with higher leverage scores are more important for one mode tensor completion (actually a matrix completion). 
In a tensor structure, we can average the element-level leverage scores over modes and treat it as the utility measurement:
% \begin{equation}
% \label{eq:lev_measure}
% {\ten{\ell}_ {{i_1}, \ldots, {i_N}}} := \sum\limits_{n = 1}^N {w_n} {\text{Fold}_n}\left( {\boldsymbol{\ell}_n} \right).
% \end{equation}
\begin{equation}
\label{eq:lev_measure}
\ten{L} := \sum\limits_{n = 1}^N {w_n} {\text{Fold}_n}\left( {\mat{L}_n} \right).
\end{equation}

\begin{comment}
\begin{figure}[!t]
    \centering
    \includegraphics[scale=0.35]{Figure/QBC_fig.png}
    \caption{Flowchart of the Query-by-Committee-based active sampling method.}
    %\zz{The color choice is very bad: the contrast is not strong enough. If you don't know how to pick the colors, then just use white background and black texts.}
    \label{fig:qbc_fig}
\end{figure}
\end{comment}

% \begin{comment}
% \begin{itemize}[leftmargin=*]
%     \item {\bf Predictive variance.} The first choice is the predicted variance from different tensor modes. Based on the solved ${\mat{X}_i}$, if we unfold it and 
%     enforcing its consistency with the observed data, we can obtain mode-$i$ low-rank approximation to $\ten{M}$:  
%     %, inspired from the classical measure, namely the disagreement among models.
%     %From the Sub-${\mat{X}_i}$ problems of our previous alternating algorithms, we can obtain a low-rank approximation tensor for one specific mode of the reconstructed tensor $\ten{M}$ via folding ${\mat{X}_i}$. 
%     %Each one is a low-rank approximation for one specific mode of the reconstructed tensor $\ten{M}$. 
%     %Therefore, after enforcing the consistency with the observed data, ${\tilde{\ten{M}}_i}$ can be seen as a mode-$i$ approximation to $\ten{M}$:
% \begin{equation} 
% \label{eq:mode_appro}
% \begin{aligned}
% & {\tilde{\ten{M}}_i} {\rm{ := }}  {{{\text{Fold}_i}(\mat{X}}_i}), \quad {\tilde{\ten{M}}_i}(\Omega) \leftarrow  \ten{T}(\Omega).
% \end{aligned}
% \end{equation}
% We define the difference tensor of each approximation ${\Delta \ten{M}_n}$ and the predictive variance tensor $\ten{V}$ as:
% \begin{equation}
% \label{eq:diff_measure}
% {\Delta \ten{M}_n} := {\tilde{\ten{M}}_i} - \mathbb{E}\left[ {\tilde{\ten{M}}} \right] 
% \end{equation}
% \begin{equation}
% \label{eq:var_measure}
% \ten{V} := \sum\limits_{i = 1}^n {{w_i}} {\left( {\Delta \ten{M}_n} \circ {\Delta \ten{M}_n} \right)}
% \end{equation}
% % with
% % \begin{equation}
% % {w_i} = \begin{cases} 
% % {{\lambda_i}} / {\sum\nolimits_i {{\lambda_i}} } & \text{if block-coordinate descent is used}\\
% % 1 / n &  \text{if ADMM is used},
% % \end{cases}   
% % \end{equation}
% %Complex version ??
% where $\circ$ denotes a Hadamard (element-wise) product, and
% ${w_i}$ is the weight associated with mode-$i$ approximation,
% ${{\tilde{\ten{M}}}_i}$. 
% The value of ${w_i}$ depends on the solver to Eq.~\reff{eq:raw_Obj}. In our implementation, we adopt ADMM solver and have $\{w_i\}_{i=1}^n = \frac{1}{n}$.
% Here, $\mathbb{E}\left[ {\tilde{\ten{M}}} \right] := \sum\limits_{i = 1}^n {{w_i}{{\tilde{\ten{M}}}_i}}$ is the expectation of all $n$ mode approximations.
% % \begin{equation}
% % \mathbb{E}\left[ {\tilde{\ten{M}}} \right] := \sum\limits_{i = 1}^n {{w_i}{{\tilde{\ten{M}}}_i}}.     
% % \end{equation}
% Among the $n$ mode approximation tensors $\left\{{\tilde{\ten{M}}_i}\right\}\nolimits_{i=1}^n$, some of the entries are estimated to be the same (\eg~the observed data) or similar (with small variance), while some other entries are estimated to be very different (with large variance).
% Thus we can treat $\ten{V}$ as a measure of disagreement. 
% \begin{lemma}
% Let ${\mu}$ be the sum of all elements of the predictive variance tensor
% $\mu:= \|{\rm vec}(\ten{V}) \|_1 = \sum\limits_{i = 1}^n {{w_i}} {\left\| {\Delta \ten{M}_n} \right\|_{\rm F}^2}$. Denote ${\mu_i}$ be the mode-$i$ approximation error: ${\mu_i}=\left\|\ten{M} - {\tilde{\ten{M}_n}} \right\|_{\rm F}^2$, and ${\mu _{\rm rec}}$ be the reconstruction error of the whole data set: $\mu _{\rm rec}=\left\|\ten{M}-\mathbb{E}\left[ {\tilde{\ten{M}}} \right] \right\|_{\rm F}^2$, then we have
% \begin{equation}
% \label{eq:relation_err_var}
% {\mu _{\rm rec}} = \sum\limits_{i = 1}^n {w_i}{\mu_i } - \mu.
% \end{equation}
% \end{lemma}
% \begin{comment}
% \begin{proof}
% Given two tensors $\ten{A}$ and $\ten{B}$ which are of the same size, we have $\|\ten{A} - \ten{B}\|_{\rm F}^2 = \|\ten{A}\|_{\rm F}^2 + \|\ten{B}\|_{\rm F}^2 - 2 \| {\rm {vec}}(\ten{A} \circ \ten{B})\|_1$. Eq.~\eqref{eq:relation_err_var} is obtained by applying such an expansion on $\mu$, $\mu_i$ and $\mu _{\rm rec}$.
% \end{proof}
% \end{comment}
% The approximation results of different modes gradually converge to the same one as more samples are observed. When the tensor is fully sampled, both $\mu$ and $\mu_{\rm rec}$ approach zero.
% Heuristically, $\mu_{\rm rec}$ decreases quickly when a sample with the highest predictive variance is selected. 

% \item  {\bf Leverage score.} Another possible quality measurement $u$ is the leverage score. It comes from the incoherence property of a matrix~\cite{candes2009exact}: a low-rank matrix can be recovered via nuclear norm minimization if it satisfies the incoherent property.
% %, which means that the theory xxx (matrixsampling2017.pdf)
% Given the singular value decomposition (SVD) of a rank-$r$ matrix $\mat{A}= \mat{U}\mat{\Sigma} {\mat{V}^H} \in {\mathbb{C}^{{n_1}\times{n_2}}}$, 
% %\hzc{Check the generalization in complex number}
% the left and right leverage scores of a matrix are defined as:
% \begin{equation}
% \begin{array}{l}
% {\mat{l}(i)} := \frac{n_1}{r}{\left\| {{\mat{U}^T}{\mat{e}_i}} \right\|^2_2},\quad i = 1,2,\ldots,{n_1}, \\
% {\mat{r}(j)} := \frac{n_2}{r}{\left\| {{\mat{V}^T}{\mat{e}_j}} \right\|^2_2},\quad j = 1,2,\ldots,{n_2}.
% \end{array}
% \end{equation}
% %The leverage scores can be also estimated from a partially observed matrix~\cite{eftekhari2018mc2}. 
% Leverage scores measure the coherence of rows/columns with coordinate directions.
% Generally, the rows/columns with larger left/right scores are more informative.
% For the mode-$k$ unfolded matrix of a tensor, we can perform SVD and calculate its left and right leverage scores as $\mat{l}_k$ and $\mat{r}_k$ respectively, then the element-level leverage score of a sample $\left(i,j \right)$ in mode $k$ is defined as:
% \begin{equation}
% \label{eq:mode_lev_measure}
% {{\mathbf{\ell}_k} \left(i,j\right)}: = {\mat{l}_k(i)} \times {\mat{r}_k(j)},\quad k=1,2,\ldots,n.
% \end{equation}
% %It is reasonable to assume that the samples with higher leverage scores are more important for one mode tensor completion (actually a matrix completion). 
% In a tensor structure, we can average the element-level leverage scores over modes and treat it as the utility measurement:
% \begin{equation}
% \label{eq:lev_measure}
% {\ten{\ell}_ {{i_1}, \ldots, {i_n}}} := \sum\limits_{i = 1}^n {w_i} {\text{Fold}_i}\left( {\mat{\ell}_i} \right).
% \end{equation}
% \end{itemize}
% \end{comment}
 
Based on the above two measurements, we propose four greedy methods for our active tensor sampling as follows. Since the sampling performance is problem-dependent, we can not conclude the best one for an arbitrary data set. But they all perform well in our numerical experiments.
%\hzc{The leverage score is based on input? Then what if non-uniform sampling???}
\begin{itemize}[leftmargin=*]

\item \textbf{Method 1 (Var):}  
We take the utility measurement $u$ as the variance among different modes [Eq.~\reff{eq:var_measure}]. 
%The variance depends on the difference among various modes, therefore this method is driven by model disagreement.

\item \textbf{Method 2 (Lev):} 
We take the utility measurement $u$ as the (weighted) average leverage scores [Eq.~\reff{eq:lev_measure}]. 
%The leverage score depends on the incoherent structure of the output mode approximations, hence this method is more driven by the problem structure.

\item \textbf{Method 3 / 4 (Var + Lev/ Var $\times$ Lev):} We take the utility measurement $u$ as the sum/ Hadamard product of the normalized variance [Eq.~\reff{eq:var_measure}] and the leverage scores [Eq.~\reff{eq:lev_measure}]. 

% \item \textbf{Method 3 (Var + Lev):} We take the utility measurement $u$ as the sum of the normalized variance [Eq.~\reff{eq:var_measure}] and the leverage scores [Eq.~\reff{eq:lev_measure}]. 
% %This method is driven by both the model disagreement and the problem structure.

% \item \textbf{Method 4 (Var $\times$ Lev):} We take the utility measurement $u$ as the Hadamard product of the normalized variance [Eq.~\reff{eq:var_measure}] and the leverage scores [Eq.~\reff{eq:lev_measure}].
\end{itemize}
\begin{figure*}[t]
    \centering
    \includegraphics[width=6.6in]{Figure/fig_3d_act.eps}
    \caption{Reconstruction results of different adaptive sampling methods. The proposed methods all outperform the existing Ada\_Coh and random methods. Method 1 (Var) is the most suitable one in this example.} 
    \label{fig:combine_act}
\end{figure*}

\subsection{Sampling under Pattern Constraint}
\label{sec:pattern_sample}
Now we show how to pick the samples subject to some pattern constraints. 
Suppose the unobserved $k$-space data is partitioned into $P$ patterns $\{\Pi_i\}_{i=1}^P$, 
we should sample a certain pattern $\Pi_i$ rather than just one element.
For example, in a Cartesian sampling, the pattern ${\Pi_i}$ is a rectilinear sampling, \ie~a full column or row in a $k$-space matrix (${k_x}$-${k_y}$).

Since our utility measurements are calculated element-wisely in the Query-by-Committee, they can be easily applied to any sampling pattern by summing the utility measurement over all elements included in the pattern. 
Consequently, we have a pattern-wise measurement:
\begin{equation}\label{eq:pattern_calculate}
u\left( \Pi_i \right) = \begin{matrix} \sum_{\xi \in \Pi_i} {u\left( \xi \right)} \end{matrix}, \quad i = 1, 2, \ldots, P.
\end{equation}
%where $\xi$ denotes a sample in the pattern $\Pi_i$.
As a result, the observation set can be updated as $\Omega \leftarrow \Omega \cup \argmax_{\Pi_i}~u\left( {\Pi_i} \right) $. 
Without any pattern constraints, Eq,~\reff{eq:pattern_calculate} will degenerate to an element-wise measurement. 
%Therefore, our pattern-wise measurements are suitable for both Cartesian and non-Cartesian sampling or some other special patterns in MRI.

In practical implementations, the active learning algorithm can be easily extended to a batch version via selecting samples with the top-$K$ utility measurement. We can stop the algorithm when the algorithm runs out of a sampling budget. Note that beyond MRI reconstruction, the proposed active learning method is suitable for various tensor completion applications with different pattern constraints. The only requirement is that the low-rank tensor completion algorithms model the (multilinear) Tucker rank.
% adding in batch
%In practical implementations, our active learning algorithm can be easily extended to a batch version. Instead of selecting one most informative sample or pattern, a batch of samples or patterns with the top-$P$ highest utility are chosen and added into the observation set, where $P$ is a batch size. 
%We can stop the algorithm when a pre-specified reconstruction accuracy is achieved or the algorithm runs out of a sampling budget. 

\begin{comment}
The complete active tensor reconstruction algorithm is summarized in Algorithm~\ref{alg:act_framework}. 
\begin{algorithm}[t]
  \caption{The comprehensive active tensor completion framework.}
  \label{alg:act_framework}
  \KwIn{Initial setting for Alg.~\ref{alg:alt_solver}, batch size $P$, active sampling method, and sampling pattern constraint} %\#}
  %and minimal step size $\Delta $
  \KwOut{Reconstructed tensor $\ten{M}$}
  \textbf{Step 1:} Run Alg.~\ref{alg:alt_solver} as initialization\\
  \textbf{Step 2:} Calculate element-wise utility measurement based on adopted sampling method\\
%   \If{\text{Strategy 1}}
%   {
%   %\For{$i= 1,2, \ldots ,n$}
%   %{
%   %Calculate mode approximation via Eq.~\reff{eq:mode_appro}\\
%   %}
%   Calculate utility measurement via Eq.~\reff{eq:var_measure}.
%   }
  
%     \If{\text{Strategy 2}}
%   {
%   \For{$i= 1,2, \ldots ,n$}
%   {
%   Calculate mode leverage scores via Eq.~\reff{eq:mode_lev_measure}\\
%   }
%   Calculate utility measurement via Eq.~\reff{eq:lev_measure}.
%   }
  
%     \If{\text{Strategy 3}}
%   {
%   \For{$i= 1,2, \ldots ,n$}
%   {
%   %Calculate mode approximation via Eq.~\reff{eq:mode_appro}\\
%   Calculate mode leverage scores via Eq.~\reff{eq:mode_lev_measure}\\
%   }
%   Calculate utility measurement via the combination of normalized Eq.~\reff{eq:var_measure} and~\reff{eq:lev_measure}.
%   }
%   %Add ${s}_{batch}$ samples with largest utility into the observation set\\
%   \For{${j}= 1,2, \ldots ,{n_{batch}}$}
  {
  %\% Shape of sample pattern is adjustable by different shape constraints\\
      \textbf{Step 3:} Select $P$ patterns based on pattern-wise utility measurement [Eq.~\reff{eq:pattern_calculate}]\\ %\quad \% Add samples \\
  \textbf{Step 4:} Rerun tensor completion algorithm (Alg.~\ref{alg:alt_solver}).
  \textbf{Step 5:} Check convergence. If not, back to step 2.
  }
\end{algorithm}
\end{comment}

\begin{comment}
\subsection{Method Analysis}
%0. Query-by-committee
\begin{lemma}
%Denote ${\mu}$ as the weighted summation over element-wise difference [Eq.~\reff{eq:diff_measure}] of all modes:
Denote ${\mu}$ as the sum of all elements of the predictive variance tensor [Eq.~\eqref{eq:var_measure}]
$\mu:= \|{\rm vec}(\ten{V}) \|_1 = \sum\limits_{i = 1}^n {{w_i}} {\left\| {\Delta \ten{M}_n} \right\|_{\rm F}^2}$, 
then we have:
\begin{equation}
\label{eq:relation_err_var}
{\mu _{\rm rec}} = \sum\limits_{i = 1}^n {w_i}{\mu_i } - \mu.
\end{equation}
Here ${\mu _{\rm rec}}$ is the reconstruction error of the whole data set $\mu _{\rm rec}=\left\|\ten{M}-\mathbb{E}\left[ {\tilde{\ten{M}}} \right] \right\|_{\rm F}^2$, and ${\mu_i}$ is the mode-$i$ approximation error ${\mu_i}=\left\|\ten{M} - {\tilde{\ten{M}_n}} \right\|_{\rm F}^2$.
\end{lemma}
\begin{proof}
Given two tensors $\ten{A}$ and $\ten{B}$ which are of the same size, we have $\|\ten{A} - \ten{B}\|_{\rm F}^2 = \|\ten{A}\|_{\rm F}^2 + \|\ten{B}\|_{\rm F}^2 - 2 \| {\rm {vec}}(\ten{A} \circ \ten{B})\|_1$. Eq.~\eqref{eq:relation_err_var} is obtained by applying such an expansion on $\mu$, $\mu_i$ and $\mu _{\rm rec}$.
\end{proof}

The approximation results of different modes converge gradually to the same one as more data samples are observed. When the tensor is fully sampled, both the sum of predictive variance $\mu$ and reconstruction error $\mu_{\rm rec}$ approach zero.
%When the variance comes to zero (i.e. the data set is fully sampled), the error will be zero.  
% As shown in Figure~\ref{fig:mode_converg}, the different mode approximations will converge to the same model gradually with more observations.  
%See from Eq.~\reff{eq:relation_err_var}, the good samples should decrease the total variance quickly. 
Heuristically, $\mu$ decreases quickly when some informative samples are selected. This is consistent with our sampling Method 1 which selects new samples with the highest predictive variance greedily. 
%1. ensemble learning
Similar formulations and ideas have been explored used in some other tasks, such as ensemble-based regression~\cite{brown2005managing,mendes2012ensemble} and surrogate modeling~\cite{fuhg2019adaptive,liu2018survey}, where one improves the diversity of training data to improve the performance of some output estimators or surrogate models. 
%2. input, output information (included into strategies)
% Or numerical, structure information

\end{comment}



==> ICIP'21_Active_tensor_MRI/conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}
In this paper, we have presented a tensor-format active sampling model for reconstructing high-dimensional low-rank MR images. 
The proposed $k$-space active sampling approach is based on the Query-by-Committee method. 
It can easily handle various pattern constraints in practical MRI scans. 
%% Numerical results
Numerical results have shown that the proposed active sampling methods outperform the existing matrix-coherence-based adaptive sampling method. 
%Given the same sampling initialization, our active sampling methods have achieve up to $20\times$ sample reduction compared with a randomized sampling. 
%% Future work
In the future, we will extend the reconstruction to an online setting and verify it on more realistic MRI data. 

% \section*{Acknowledgment}
% This work was supported by NSF CCF No. 1763699 and NSF CAREER Award No. 1846476.


==> ICIP'21_Active_tensor_MRI/introduction.tex <==
\section{Introduction}
\label{sec: intro}
%Magnetic resonance imaging (MRI) is widely used in clinical diagnosis and brain science. In order to reduce the MRI scanning time and cost, it is highly desirable to accurately reconstruct MRI from some undersampled data. 
Magnetic resonance imaging is a major medical imaging modality, which is widely used in clinical diagnosis and neuroscience. Due to the limited imaging speed, it is often highly desirable to speed up its imaging process. 
%Two mathematical approaches can help achieve this goal. 
%Firstly, given some obtained samples, one can design a better image model to achieve higher accuracy.
%Alternatively, one can employ experimental design or active sampling to reduce the sampling cost of a specific reconstruction model. 
A lot of image models have been proposed to accelerate MR imaging, including sparsity-constrained~\cite{lustig2007sparse}, low-rank-constrained~\cite{liang2007spatiotemporal,lingala2011accelerated,zhao2012image}, data-driven, learning-based approaches, etc~\cite{ravishankar2019image}. 
Most of these methods recover MRI data with matrix computational techniques. 
They either focus on 2-D MRI problems or reshape the high-dimensional MRI data into a matrix and then solve the problem using matrix-based techniques. 
%such as formulating low-rank Hankle matrix~\cite{ye2016compressive}, local low-rank modeling~\cite{haldar2013low}, compressive sensing~\cite{ye2019compressed,zhao2015accelerated}, matrix completion~\cite{otazo2015low} and so forth.

As a multi-dimensional generalization of matrix computation, tensor computation has been recently employed in MRI due to its capability of handling high-dimensional data~\cite{yu2014multidimensional,trzasko2013unified}. 
In many applications, MRI data sets naturally have a higher physical dimension. 
%Examples include dynamic MRI, parallel MRI, multi-contrast MRI, and so forth~\cite{trzasko2013unified,christodoulou2018magnetic,banco2016sampling,yu2014multidimensional,cheng2017comprehensive,huang2014fast}.
In these cases, tensors often better capture the hidden high-dimensional data pattern, achieving better reconstruction performance~\cite{he2016accelerated,kanatsoulis2019tensor}.

The quality and efficiency of an MRI reconstruction also highly depend on the sampling method.
Practical samples are measured in the spatial frequency domain of an MR image, often known as $k$-space.
Some adaptive sampling techniques have been proposed for matrix-format MR imaging based on compressive sensing or low-rank models~\cite{8632928,levine2017fly}. 
The experimental design methodologies include the Bayesian model~\cite{seeger2010optimization}, learning-based framework~\cite{gozcu2018learning,zhao2018optimal}, %self-supervised framework~\cite{jin2019self}, 
and so forth. Adaptive samplings may also be considered for streaming data~\cite{mardani2015subspace}. 

However, active sampling has not been explored for fast MR imaging with low-rank tensor models. 
Beyond the application of MR imaging, there are also limited works of adaptive sampling for tensor-structured data. 
Existing works mainly rely on the matrix coherence property~\cite{krishnamurthy2013low,liu2015adaptive}. %deng2020network  
They need to reshape the tensor to a matrix or can only apply on a 3-D tensor. 
Additionally, the practical MRI sampling is usually subject to some pattern constraints, like a Cartesian line sampling. 
Few papers have considered the pattern constraints caused by the practical MRI sampling.
Therefore, designing an active sampling method for tensor-structured data under certain pattern constraints is an important and open problem.

\textbf{Paper contributions.}
This paper presents an active sampling method for accelerating high-dimensional MR Imaging with low-rank tensors. 
% Firstly, We model the MRI reconstruction as a low-rank tensor completion problem. 
% Then a Query-by-Committee method is presented to search for the most informative sample adaptively. Making use of the special tensor structure, the approximations towards the unfolding matrices naturally consist the committee. The measurement of sample quality can be the predictive variance, averaged leverage scores, or the combination of them. 
% The proposed sampling method can be easily extended to fit various kinds of sampling patterns in MR imaging. However, the proposed sampling methods can be also applied broadly beyond MRI reconstruction.
% We demonstrate the model in a 3D MRI data set with a Cartesian line sampling pattern. Numerical results show that our proposed methods outperform the existing matrix coherence based method.
Our specific contributions include:
\begin{itemize}[leftmargin=*]
    \item Novel active sampling methods for low-rank tensor-structured MRI data. A Query-by-Committee method is used to search for the most informative sample adaptively. Making use of the special tensor structure, the approximations towards the unfolding matrices naturally forms a committee. The sample quality is measured by the predictive variance, averaged leverage scores, or their combinations.
    \item Extending the sampling method to handle some pattern constraints in MR imaging. Our proposed sampling method itself can be applied broadly beyond MRI reconstruction.
    \item Numerical validation on an MRI example with Cartesian sampling. Numerical results show that the proposed methods outperform the existing tensor sampling methods.
\end{itemize}

\begin{comment}
\begin{figure}[t]
    \centering
    \includegraphics[width=3.3in]{Figure/masks.eps}
    \caption{Some popular $k$-space MRI sampling patterns: (a) Non-Cartesian sampling in a radial trajectory; (b) Fully sampled central region and randomly non-Cartesian sampled non-central region; (c) Fully sampled central region and randomly Cartesian sampled non-central region; (d) Randomly Cartesian sampling.}
    \label{fig:sample_pattern}
\end{figure}
\end{comment}

==> ICIP'21_Active_tensor_MRI/numerical_result.tex <==
\section{Numerical results}
\label{sec:numerical_results}
In this section, we validate our active sampling methods on a low-rank tensor-format brain data set with the size $256 \times 256 \times 256$. Our codes are implemented in MATLAB and run on a computer with 2.3GHz CPU and 16GB memory. 
%Our algorithm is implemented in MATLAB and run on a laptop with 2.3GHz CPU and 16GB memory.
\begin{figure}[t]
    \centering
    \includegraphics[width=1\columnwidth]{Figure/fig_rec.eps}
    \caption{One slice of the reconstructed data.}
    \label{fig:Spatial}
\end{figure}

% \textbf{Data set.} 
% We use a 3D brain data with the size $256 \times 256 \times 256$to demonstrate the proposed active tensor completion model. 
% We use a 3D-spatial MRI data\footnote{Available at http://www.cse.yorku.ca/~mridataset/} to demonstrate the proposed active tensor completion model. 
% This data set has some cardiac MR images acquired from 33 subjects. 
% The sequence of each subject consists of 20 time frames and 8-15 slices along the third spatial axis~\cite{andreopoulos2008efficient}.
% We select one frame of one subject with size $256 \times 256 \times 10$ for validation here.
%Note that our model can be easily applied to 4-D or 5-D MRI data, such as ${k_x}$-${k_y}$-z-coil or ${k_x}$-${k_y}$-z-coil-contrast data sets.

{\bf Baselines for Comparisons.} 
We reconstruct the tensor-structured data via adopting the proposed active learning methods, a matrix-coherence-based adaptive tensor sampling method (denoted as Ada\_Coh)~\cite{krishnamurthy2013low}, and a random sampling method. In Ada\_Coh~\cite{krishnamurthy2013low}, the sampling is driven by the coherence of one mode matricization of a tensor. Our Method 2 (Lev) can be seen as its generalization via taking consideration of the interactions among different modes. 

\textbf{Sampling Patterns.} In this example, the $k$-space data is scanned continuously as a fiber in the Cartesian coordinate. In each spatial slice, we initialize with a fully sampled center and randomly sampled non-central regions. The sample pattern of the candidate samples is a fiber in the $k$-space, which is obtained via fixing all but one index of the tensor.

\textbf{Evaluation metrics.}
Our methods sample and predict $k$-space data, and the final reconstruction needs to be visualized in the image space. Therefore, we choose the evaluation metrics from both spaces. 
In the $k$-space, the accuracy is measured by the relative mean square error evaluated over the fully-sampled $k$-space data (denoted as $k$-test). 
In the image space, we use the signal to error ratio (SER) and peak signal to noise ratio (PSNR) as our metrics.
% : 
% \begin{equation}
% \begin{aligned} 
% &{\rm {SER}} :=  - 10{\log _{10}}\frac{{{{\left\| {{\ten{I}_{\rm {res}}} - {\ten{I}_{\rm {full}}}} \right\|}_F}}}{{{{\left\| {{\ten{I}_{\rm {full}}}} \right\|}_F}}}  \\
% &{\rm {PSNR}} := 20{\log _{10}}\frac{{\max \left( {{\ten{I}_{\rm {res}}}} \right)}}{{\sqrt { {\rm {MSE}}(\ten{I})} }}.
% \end{aligned}
% \end{equation}
% Here $\ten{I}_{\rm {res}}$ and $\ten{I}_{\rm {full}}$ denote the reconstructed and true image space data, and ${{\rm {MSE}}(\ten{I})}$ is their mean square error. 

\textbf{Results Summmary.} The initial sampling mask is generated with a sampling ratio of 23.14\%, including a 14.45\% fully sampled center. In active sampling, each sampling batch includes 1000 fibers, and we select a total of 10 batches sequentially. 
%We perform the experiments via adopting the proposed active learning methods, a adaptive sampling method based on matrix coherence (denoted as Ada\_Coh)~\cite{krishnamurthy2013low}, and a random sampling method.
Fig.~\ref{fig:combine_act} plots the $k$-test, SER and PSNR as the sampling ratio increases. 
All proposed active sampling methods can significantly improve the evaluation metrics and outperform the existing Ada\_Coh and random samplings. We choose Method 1 (Var) for the further comparison. Fig.~\ref{fig:Spatial} shows one slice of the reconstructed MRI data. The evaluations of the whole data set are shown in Table~\ref{tab:evaluation}, where the proposed method has a higher reconstruction accuracy.
%From Table~\ref{Tb:needed_sample}, we can see that our proposed active tensor completion achieves up to 20 sample reduction when achieving the similar performance of a random sampling method.
\begin{table}[t]
\centering
\caption{Evaluations on the whole data set.}
\label{tab:evaluation}
\begin{tabular}{cccc}
\toprule
 Sampling method    & $k$-test (\%) & SER (dB) & PSNR (dB)  \\
\midrule
    Random & 3.85      & 14.56      & 29.36       \\
 Ada\_Coh~\cite{krishnamurthy2013low}  & 1.52  & 18.56 &  33.67      \\
\textbf{Proposed} & \textbf{0.85}  & \textbf{21.22} &  \textbf{35.84}     \\
\bottomrule
\end{tabular}
\end{table}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{comment}
\begin{table*}[t]
\centering
\caption{The number of added samples to achieve the expected metrics change.}
\label{Tb:needed_sample}
\begin{tabular}{cccccccc}
\toprule
Metric & Change & Var &Lev & Var+Lev & Var$\times$Lev & Rand & Reduction\\
\midrule
$k$-test & 0.1085$\to$0.076
& \textbf{$<$0.31\%}  & $<$0.61\% & $<$0.31\% & $<$0.31\% & 6.1\%  & 20x \\
SER (dB)& 10.29$\to$12.13         
& \textbf{$<$0.31\%}  & $<$0.61\% & $<$0.31\% & $<$0.31\% & 6.1\%  & 20x \\
PSNR (dB)& 32.74$\to$34.03         
& \textbf{$<$0.31\%}  & $<$0.31\% & $<$0.31\% & $<$0.31\% & 6.1\%  & 20x \\
\bottomrule
\end{tabular}
\end{table*}
\end{comment}
\begin{comment}
\begin{figure}[t]
\centering
\subfigure{
\begin{minipage}[t]{0.48\linewidth}
\centering
\includegraphics[width=1\columnwidth]{Figure/3D_spatial/initial_err.eps}
%\caption{fig2}
\end{minipage}
}%
\subfigure{
\begin{minipage}[t]{0.48\linewidth}
\centering
\includegraphics[width=1\columnwidth]{Figure/3D_spatial/rand_err.eps}
%\caption{fig2}
\end{minipage}
}%

\\
\subfigure{
\begin{minipage}[t]{0.48\linewidth}
\centering
\includegraphics[width=1\columnwidth]{Figure/3D_spatial/ada_coh_err.eps}
%\caption{fig2}
\end{minipage}
}%
\subfigure{
\begin{minipage}[t]{0.48\linewidth}
\centering
\includegraphics[width=1\columnwidth]{Figure/3D_spatial/tensor_err.eps}
%\caption{fig2}
\end{minipage}
}%
% \\
% \subfigure{
% \begin{minipage}[t]{0.48\linewidth}
% \centering
% \includegraphics[width=1\columnwidth]{Figure/3D_spatial/matrix.eps}
% %\caption{fig2}
% \end{minipage}
% }%
% \subfigure{
% \begin{minipage}[t]{0.48\linewidth}
% \centering
% \includegraphics[width=1\columnwidth]{Figure/3D_spatial/matrix_err.eps}
% \end{minipage}
% }%
\centering
\caption{Reconstruction error.
The initial reconstruction: SER=10.15dB and PSNR=30.19dB.
The reconstruction with random sampling: SER=10.82dB and PSNR=31.22dB.
The reconstruction with Ada\_Coh sampling: SER=13.77dB and PSNR=34.55dB.
The reconstruction with proposed sampling Method 4 (Var $\times$ Lev): SER=15.17dB and PSNR=36.45dB. \hzc{Sorry, the experiments are still running, but will finish them.}
}
\label{fig:Spatial_rec}
\end{figure}

\end{comment}
\begin{comment}
\begin{figure*}[!t]
    \centering
    \includegraphics[width=2\columnwidth]{Figure/recon.png}
    \caption{Reconstruction of the fused multi-coil data.
    The initial observation: SER=11.50dB and PSNR=32.83dB.
    %The initial matrix-structure reconstruction: SER=12.24dB and PSNR=34.40dB.
    The tensor-structure reconstruction with adaptively adding samples via Method 2 (Lev): SER=12.27dB and PSNR=35.78dB for the initial; SER=19.31dB and PSNR=42.83dB for adding 125 fibers; SER=25.13dB and PSNR=48.64dB for adding 250 fibers.
    The tensor-structure reconstruction with adaptively adding samples randomly: SER=12.27dB and PSNR=35.78dB for the initial; SER=13.17dB and PSNR=35.11dB for adding 125 fibers; SER=14.52dB and PSNR=36.47dB for adding 250 fibers}
    \label{fig:coil_rec}
\end{figure*}
\end{comment}






==> ICIP'21_Active_tensor_MRI/preliminary.tex <==
\section{Background}
\label{sec:preliminaries}
%In this paper, all the vector, matrix, tensor...
\subsection{Notation}
Throughout this paper, a scalar is represented by a lowercase letter, \eg, $x$;
a vector or matrix is represented by a boldface lowercase or capital letter respectively, \eg, $\mat{x}$ and $\mat{X}$.
A tensor, which describes a multidimensional data array, is represented by a calligraphic letter. For instance, a $N$-dimensional tensor is denoted as $\ten{X} \in \mathbb{R}^{{I_1} \times {I_2}\ldots \times {I_N}}$, where ${I_n}$ is the mode size of the $n$-th mode (or dimension). 
% Complex version?
%A vector or matrix can be seen as a special case of tensor with dimension one or three. 
An element indexed by $({i_1}, {i_2}\ldots, {i_N})$ in tensor $\ten{X}$ is denoted as $x_{{i_1}{i_2}\ldots{i_N}}$. 
A tensor Frobenius norm is defined as $\left\|\ten{X} \right\|_F := \sqrt{\sum\limits_{{i_1},{i_2},\ldots,{i_N}}({x_{{i_1}{i_2}\cdots{i_N}}})^2}$. 
A tensor $\ten{X} \in \mathbb{R}^{{I_1} \times {I_2}\cdots \times {I_N}}$ can be unfolded into a matrix along the $n$-th mode/dimension, denoted as ${\text{Unfold}_n}(\ten{X}):={\mat{X}_{(n)}} \in \mathbb{R}^{{I_n}\times {{I_1}\cdots{I_{n-1}}{I_{n+1}}\cdots{I_{N}} }}$.  
Conversely, folding the $n$-mode matrization back to the original tensor is denoted as ${\text{Fold}_n}({\mat{X}_{(n)}}):=\ten{X}$.

\subsection{Tensor-Format MRI Reconstruction}
In tensor completion, one aims to predict a whole tenser given only partial elements of the tensor, which is similar with matrix completion. 
In matrix cases, one often uses the nuclear norm ${\left\|  \cdot  \right\|_*}$ (sum of singular values) as a surrogate of a matrix rank, and seeks for a matrix with the minimal nuclear norm.
Exactly computing the tensor rank is NP-hard~\cite{hillar2013most}.
A popular heuristic surrogate of the tensor (multilinear) Tucker rank is the generalization of matrix nuclear norms~\cite{liu2012tensor}: 
% \begin{equation}\label{eq:ten_nuclear}
% {\left\| \ten{X} \right\|_*} = \sum\limits_{n = 1}^N {{\alpha _n}{{\left\| {{\mat{X}_{\left( n \right)}}} \right\|}_* }},
% \end{equation}
\begin{equation}\label{eq:ten_nuclear}
{\left\| \ten{X} \right\|_*} = \sum\limits_{n = 1}^N {{{\left\| {{\mat{X}_{\left( n \right)}}} \right\|}_* }},
\end{equation}
%where $\{{\alpha _n}\}^N_{n=1}$ are the weights, satisfying ${\alpha _n}>0$ and $\sum\nolimits_{n = 1}^N {{\alpha _n}}  = 1$. 
Then the tensor completion problem can be formulated as minimizing Eq.~\reff{eq:ten_nuclear} given existing observations.

\begin{comment}
Consequently, a low-rank tensor completion problem can be formulated as:
\begin{equation}
\label{eq:min_lr_ten}
\begin{aligned}
\mathop {\min }\limits_{\ten{X}} \quad & {\sum\limits_{n = 1}^N {{\alpha _n}{{\left\| {{\mat{X}_{\left( i \right)}}} \right\|}_* }}} \\  
\st \quad & {\ten{X}_\Omega } = {\ten{T}_\Omega },
\end{aligned}
\end{equation}
where $\ten{T}$ is the original tensor, and $\Omega$ is its observation set.
%For more detail about tensor algebra, we refer readers to a nice overview paper~\cite{kolda2009tensor}. 
%what is tensor, Fold function, tensor rank
%what is tensor completion (low-rank minimization) formulation
\end{comment}

% \subsection{Low-Rank Tensor-Format MRI Reconstruction}
The above mode-$n$ matricization $\{{\mat{X}_{(n)}}\}^N_{n=1}$ represents the same set of data and thus are coupled to each other, which makes it hard to solve.
Therefore, we replace them with $n$ additional matrices $\{{\mat{X}_n}\}^N_{n=1}$ and introduce an additional tensor $\ten{M}$. The optimization problem can be reformulated as:
\begin{equation}\label{eq:raw_Obj}
% \begin{aligned}
% \mathop {\min }\limits_{\left\{\mat{X}_n\right\}^N_{n=1},\ten{M}} \quad & \sum\limits_{n = 1}^N {{\alpha_n}{{\left\| {{\mat{X}_n}} \right\|}_ * }}\\
% \st \quad & {\ten{M}_\Omega } = {\ten{T}_\Omega } \; \text{and}\; {\mat{X}_ n} = {\mat{M}_{(n)}},\; n = [1,N].
% \end{aligned}
\begin{aligned}
\mathop {\min }\limits_{\left\{\mat{X}_n\right\}^N_{n=1},\ten{M}} \quad& \sum\limits_{n = 1}^N {{{\left\| {{\mat{X}_n}} \right\|}_ * }}\\
\st \quad&{\mat{X}_ n} = {\mat{M}_{(n)}},\; n = 1,2,\ldots,N,\\
 & {\ten{M}_\Omega } = {\ten{T}_\Omega }, 
\end{aligned}
\end{equation}
where $\ten{M}$ is the reconstructed $k$-space tensor, $\mat{M}_{(n)}$ is the $n$-th mode matricization of $\ten{M}$, $\ten{T}$ is the fully sampled $k$-space tensor, and $\Omega$ is the observation set.
If the MRI data is known to hold some additional structure, we can further modify the imagining model, like a low-rank plus sparsity model~\cite{otazo2015low}. %~\cite{roohi2017multi}
Eq.~\reff{eq:raw_Obj} can be efficiently solved via some alternating solvers, like the block coordinate descent and the alternating direction method of multipliers (ADMM)~\cite{liu2012tensor}. 
Essentially, we can either model the low-rankness of the $k$-space or the image space data.
We choose the former one since it enables the design of our active sampling methods in Section~\ref{sec:active_strategy}.
The additional $k$-space mode approximations $\left\{\mat{X}_n\right\}^N_{n=1}$ will be exploited to 
acquire new data.

\begin{figure}[!t]
    \centering
    \includegraphics[scale=0.38]{Figure/framework.png}
    \caption{Flowchart of the MRI reconstruction framework.}
    \label{fig:whole_framework}
\end{figure}

==> ICIP'21_Active_tensor_MRI/related_works.tex <==
\section{Related works}
\label{sec:related_works}
\par
\textbf{Tensor Methods for MRI Reconstruction:}
Tensor has been employed in the MR imaging since the ambient dimension of MRI data sets is often high. 
%lots of MRI data naturally hold a high-dimensional structure.
Yang~\etal~\cite{yang2017dynamic} showed that low-rank tensor completion with a sparsity regularizer could accelerate MRI reconstruction.
%\cite{banco2016sampling} summarized several tensor models for MRI data.
Christodoulou~\etal~\cite{christodoulou2018magnetic} applied low-rank tensor modeling for motion-resolved quantitative imaging.
The sparse transform of compressive-sensing MRI is formulated as a Tucker tensor decomposition in~\cite{yu2014multidimensional}. 
Liu~\etal~\cite{liu2018accelerated} proposed a phase-constrained low-rank model for high b-value diffusion-weighted MRI.
The theory of regular sub-Nyquist samplings for tensor completion was studied in \cite{kanatsoulis2019tensor}.
He~\etal~\cite{he2016accelerated} firstly estimated an explicit low-rank tensor subspace and reconstructed high-dimensional data via fitting the subspace. 
A locally low-rank tensor method for dynamic cardiac MRI reconstruction is proposed by Liu~\etal~\cite{liu2019dynamic}, where patch-based local structure is exploited. 
%Roohi~\etal~\cite{roohi2017multi} adopted a low-rank plus sparsity tensor structure for MRI reconstruction, but with a different optimization formulation.
Although tensor models have been exploited to enable MRI reconstruction from highly-undersampled data, this paper is the first to leverage tensor model for active sampling in MR imaging. 
%Although various tensor models have been reported for MRI reconstruction, to the best of our knowledge this paper is the first to consider adaptive sampling for tensor MRI data. 

\textbf{Experimental Design for MRI:} 
Experimental design or active sampling is an important approach to accelerate MRI reconstruction.
Seeger~\etal~\cite{seeger2010optimization} proposed a Bayesian experimental design framework by maximizing the information gain.
A learning-based method was proposed in \cite{gozcu2018learning} to select samples for compressive MRI.
Ravishankar~\etal~\cite{ravishankar2011adaptive} partitioned the sampling space and proposed an adaptive sampling pattern by moving the samples among blocks.
Zhao~\etal~\cite{zhao2018optimal} proposed an optimal experimental design to maximize the signal-to-noise ratio efficiency with estimation-theoretic bounds.
A self-supervised framework is proposed by Jin~\etal~\cite{jin2019self} to accelerate compressive MRI by considering both the data acquisition and the reconstruction process within a single deep network.
Zhang~\etal~\cite{zhang2019reducing} proposed an active acquisition model based on uncertainty reduction via introducing an evaluator network which evaluates the quality gain in reconstruction of each $k$-space measurement.

Once the MRI reconstruction is formulated as a matrix/ tensor completion problem, the experimental design becomes an active matrix/tensor completion problem. 
%Chouvardas~\etal~\cite{chouvardas2016method} adopts QBC strategy to identify informative areas of a map matrix. 
%\cite{ruchansky2015matrix} offers an active sampling according to the matrix structure from the perspective of a linear equation system.
Some researchers developed Bayesian frameworks for active matrix completion~\cite{chakraborty2013active,sutherland2013active}. 
Claude~\etal~\cite{claude2017efficient} offered an adaptive sampling method under smoothness assumption on matrix components. 
An entropy-driven approach for active matrix completion with uncertainty quantification was also proposed in~\cite{mak2017active}.

However, the active sampling for tensor completion problems is much less studied.
An adaptive tubal-sampling method is proposed for a 3D low-tubal-rank tensor completion~\cite{liu2015adaptive}, but it could not be generalized to higher-order tensors.
Krishnamurthy and Singh~\cite{krishnamurthy2013low} proposed a probabilistic sampling method to adaptively estimate and update the tensor singular subspace based on an incoherent condition. Both of them did not consider the pattern constraints in MRI sampling.
%and assumed an initialization of uniform sampling, which is infeasible in most MR images.
To the best of our knowledge, this work is the first to propose a deterministic active sampling method %for tensor MRI reconstruction with consideration of the pattern constraints in MRI measurement.
for tensor MR imaging while incorporating sampling constraint inherent in MR data acquisition process. 

%Compressive sensing MRI based on Leverage score~\cite{krahmer2013stable}.
% \par
% \textbf{Active matrix/tensor completion} Active matrix completion has been recently paid more attention by researchers.


%\textbf{L+S for MRI reconstruction:}
%Although L+S has been a classical structure in the image reconstruction field, our completion formulation is still valuable.  
% Our model extends the L+S MRI reconstruction framework~\cite{otazo2015low} to a high-dimensional $k$-space tensor case, where our target objection is direct $k$-space data. 
% Besides the MRI applications, the L+S structure is also widely used.
% Go decomposition~\cite{zhou2011godec} sets a prior setting on the matrix rank and sparsity level as the problem constraints, which is however not easy to know in the practice. 
% Robust PCA~\cite{candes2011robust} proposed an exact L+S decomposition to a matrix, but which may be not available under noise. 
% \cite{lu2016tensor} proposed a tensor robust PCA based on a special t-SVD nuclear norm, which is restricted for 3D tensor data.
% Some other papers used ADMM algorithm to solve the tensor L+S structure formulation~\cite{goldfarb2014robust,roohi2017multi}. 




==> ICIP'21_Active_tensor_MRI/tensor_completion.tex <==
\section{Low-rank Tensor-Format MRI Reconstruction}
\label{sec:ten_completion}
As shown in~\reff{eq:ten_nuclear}, $n$ mode matricization $\{{\mat{X}_{(i)}}\}^n_{i=1}$ represents the same set of data and thus are coupled to each other, which makes it hard to solve.
Therefore, we replace them with $n$ additional matrices $\{{\mat{X}_i}\}^n_{i=1}$ and introduce an additional tensor $\ten{M}$. The optimization problem can be reformulated as:
\begin{equation}\label{eq:raw_Obj}
\begin{aligned}
\mathop {\min }\limits_{\left\{\mat{X}_i\right\}^n_{i=1},\ten{M}} \quad & \sum\limits_{i = 1}^n {{\alpha_i}{{\left\| {{\mat{X}_i}} \right\|}_ * }}\\
\st \quad & {\mat{X}_ i} = {\mat{M}_{(i)}},\quad i = 1,2,\ldots,n\\
&{\ten{M}_\Omega } = {\ten{T}_\Omega }.
\end{aligned}
\end{equation}
where $\ten{M}$ is a tensor in the $k$-space; $\mat{M}_{(i)}$ is the $i$-th mode matricization of $\ten{M}$; $\ten{T}$ is the fully sampled $k$-space tensor and $\Omega$ is its observation set;
Essentially, we can model the low-rankness of both the $k$-space and image space data. 
We choose the former one since it enables the design of our active sampling methods in Section~\ref{sec:active_strategy}.
If the MRI data is known to hold some additional structure, we can further modify the imagining model by adding a regularization term, like the low rank plus sparsity model~\cite{roohi2017multi}.

Eq.~\reff{eq:raw_Obj} can be efficiently solved via some alternating solvers, like block coordinate descent and alternating direction method of multipliers (ADMM)~\cite{liu2012tensor}. 
Our proposed active sampling strategies will exploit these additional mode approximations $\left\{\mat{X}_i\right\}^n_{i=1}$ to acquire new $k$-space samples.
The complete flowchart of our MRI reconstruction framework is illustrated in Fig.~\ref{fig:whole_framework}.
\begin{figure}[!t]
    \centering
    \includegraphics[scale=0.4]{Figure/framework.png}
    \caption{Flowchart of the MRI reconstruction framework.}
    \label{fig:whole_framework}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{comment}
\subsection{Block Coordinate Descent Solver to Eq.~\reff{eq:raw_Obj}} 
The first equality constraint in Eq.~\reff{eq:raw_Obj} still makes the variables coupled to each other. To address this issue, we further relax the problem and convert it to the following one:
%To address this issue, we further relax it as:
% \begin{equation}
% {\left\| {{\mat{M}_{\left( i \right)}} - {\mat{L}_i} - {\mat{S}_{\left( i \right)}}} \right\|_F} \le {\epsilon_i}, \quad i = 1,2,\ldots,n,   
% \end{equation}
%where %${\left\|  \cdot  \right\|_F}$ is the matrix Frobenius norm and 
%${\epsilon_i}$ is a numerical threshold for approximation.
%Then the problem can be converted into the following equivalent one: 
\begin{equation} \label{eq:BCD_Obj}
\begin{aligned}
\min_\limits_{\left\{\mat{L}_i\right\}^n_{i=1},\ten{S},\ten{M}} \quad & 
\sum\limits_{i = 1}^n ({{\alpha_i}{{\left\| {\mat{L}_i} \right\|}_ * }}  + \frac{{\lambda_i}}{{2}}\left\| {{\ten{L}_ i} + {\mat{S}_{(i)}} - {\mat{M}_{(i)}}} \right\|_F^2) \\
& + {\lambda}{\left\| \mathbb{T}{\mathbb{F}^{-1}}\ten{S} \right\|_1}\\
\st \quad  &{\ten{M}_\Omega } = {\ten{T}_\Omega }
\end{aligned}
\end{equation}
where $\lambda_i$ is a fixed positive constant associated with each relaxed constraint. The resulting problem~\eqref{eq:BCD_Obj} is convex and decoupled, and it can be easily solved via a block coordinate descent (BCD) algorithm. 

The block coordinate descent method divides all variables into several groups and solves a sub-problem of each group while keeping others fixed. 
Specifically, we divide all variables into $n+2$ groups: $\left\{ {{\mat{L}_i}} \right\}_{i = 1}^n$, $\ten{S}$, and $\ten{M}$. 
%Then each group of variables can be updated with a closed-form solution during the iteration. 
In every iteration, the subproblems shown in appendix~\ref{sec:appendix_BCD} are solved with the following closed-form updates: 
\begin{itemize}[leftmargin=*]

    \item Update ${\mat{L}_i}$: 
    \begin{equation}\label{eq:BCD_L}
    {\mat{L}_i} = {\text{SVT}_{\frac{{{\alpha_i}}}{{{\lambda _i}}}}}\left( {{\mat{M}_{\left( i \right)}} -  {\mat{S}_{(i)}}} \right).
    \end{equation}
    Here $\text{SVT}(\cdot)$ denotes a singular value thresholding operator~\cite{cai2010singular}. Let $\mat{X} = \mat{U}\mat{{\Sigma }}\mat{{V^H}}$ be a singular value decomposition, then ${\text{SVT}_\tau }\left( \mat{X} \right) = \mat{U}\mat{{\Sigma _\tau }}\mat{{V^H}}$. Here $\mat{\Sigma}_\tau$ is a diagonal matrix and its $i$-th element is $ \max (\sigma_i - \tau, 0)$ with $\sigma_i$ being the $i$-th largest singular value of $\mat{X}$. 
    \item Update $\ten{S}$:
    \begin{equation}\label{eq:BCD_S}
    \ten{S} = {\mathbb{T}^{ - 1}}\left[\mathbb{F}\left( {{\Lambda _{{\lambda}}}\left( {\mathbb{T}{\mathbb{F}^{ - 1}}\left[ {\ten{M} - \frac{{\sum\nolimits_i {{\lambda_i}{\text{Fold}_i}\left( {{\mat{L}_i}} \right)} }}{{\sum\nolimits_i {{\lambda_i}} }}} \right]} \right)} \right)\right ].
    \end{equation}
    Here ${\Lambda _\lambda }\left( x \right)$ denotes a soft-thresholding operator ${\Lambda _\lambda }\left( x \right) = \frac{x}{{\left| x \right|}}\max \left( {\left| x \right| - \lambda ,0} \right)$
    where $\left|x\right|$ is the amplitude of a complex number $x$. The operator $\Lambda(\cdot)$ can be extended to a matrix or tensor case by applying it on each element. 
    
    \item Update $\ten{M}$: each element is updated as follows:
    \begin{equation}
    \label{eq:BCD_M}
    \begin{array}{l}
    {m_{{i_1} \ldots {i_n}}} = 
    \left\{{ 
    \begin{array}{cc}
    {{{\hat{m}}_{{i_1}, \ldots ,{i_n}}}}, & \text{if } {\left( {{i_1}, \ldots ,{i_n}} \right) \notin \Omega }  \\
    {{t_{{i_1}, \ldots ,{i_n}}}}, & {\text{otherwise} }
    \end{array} } \right. \\
    \text{with tensor }   {\hat{\ten{M}}} ={ {\frac{{\sum\nolimits_i {{\lambda_i}{\text{Fold}_i}\left( {{\mat{L}_i}} \right)} }}{{\sum\nolimits_i {{\lambda_i}} }} + \ten{S}. }} 
 \end{array}
    \end{equation}
    Here $t_{i_1 i_2 \cdots i_n}$ denotes one element of $\ten{T}$.
\end{itemize}



% Every iteration of the BCD solves the following sub-problems: 
% %\zz{You didn't fix my comments in the email.}
% \begin{itemize}

%     \item Sub-${\mat{L}_i}$ problem: fixing $\ten{S}$ and $\ten{M}$, we update $\{ \mat{L}_i\}$ by solving the following problem:
% \begin{equation}
% \label{eq:sub-L}
% \begin{array}{ll}
% \mathop {\min } \limits_{\{\mat{L}_i\}} & \sum\limits_{i = 1}^n {{\alpha_i}{{\left\| {{\mat{L}_i}} \right\|}_*}}  + \frac{{{\lambda_i}}}{2}\left\| {{\mat{L}_i} + {\mat{S}_{(i)}} - {\mat{M}_{(i)}}} \right\|_F^2 \\
% & \equiv \sum\limits_{i = 1}^n \frac{1}{2}\left\| {{\mat{L}_i} + {\mat{S}_{(i)}} - {\mat{M}_{(i)}}} \right\|_F^2 + \frac{{{\alpha_i}}}{{{\lambda_i}}}{\left\| {{\mat{L}_i}} \right\|_*}.
% \end{array}
% \end{equation} 
% To solve Eq.~\reff{eq:sub-L}, we need to use a singular value thresholding (SVT) operator~\cite{cai2010singular}.
% Let $\mat{X} = \mat{U}\mat{{\Sigma }}\mat{{V^H}}$ be the singular value decomposition for $X$. Then the singular value thresholding operator ${\text{SVT}_\lambda }\left( \mat{X} \right)$ is defined as ${\text{SVT}_\lambda }\left( \mat{X} \right) = \mat{U}\mat{{\Sigma _\lambda }}\mat{{V^H}}$, where $\mat{\Sigma _\lambda} = \text{diag}(\max (\sigma_i - \lambda, 0))$ and $\sigma_i$ is the $i$th largest singular value. 
% Note that here the matrix $\mat{X}$ is complex, thus the conjugate transpose is used. 
% We can easily compute the optimal ${\mat{L}_i}$ as:
% \begin{equation}
% {\mat{L}_i} = {\text{SVT}_{\frac{{{\alpha_i}}}{{{\lambda _e}}}}}\left( {{\mat{M}_{\left( i \right)}} -  {\mat{S}_{(i)}}} \right).
% \end{equation}

% \item Sub-$\ten{S}$ problem: we fix $\{ \mat{L}_i\}$ and $\ten{M}$, then update $\ten{S}$ by solving
% \begin{equation}
% \label{eq:sub-S}
% \begin{array}{ll}
% \mathop {\min }\limits_{\ten{S}} & \sum\limits_{i = 1}^n \frac{{{\lambda_i}}}{2}\left\| {{\mat{L}_i} + {\mat{S}_{(i)}} - {\mat{M}_{(i)}}} \right\|_F^2 + {\lambda}{\left\| {\mathbb{T}{\mathbb{F}^{-1}}\ten{S}} \right\|_1}\\
% \end{array}
% \end{equation}
% To solve Eq.~\reff{eq:sub-S}, a soft-thresholding operator 
% ${\Lambda _\lambda }\left( x \right) = \frac{x}{{\left| x \right|}}\max \left( {\left| x \right| - \lambda ,0} \right)$ 
% is defined, where $\left|x\right|$ is the amplitude of a complex number $x$. 
% %\zz{(Please consider using another notation for the soft thresholding operator, because it's very similar to the aquisition operator in Eq. (4).) }
% The operator $\Lambda$ can be generalized to a tensor case when we apply it to each entry.
% The solution of Eq.~\reff{eq:sub-S} is given by
% \begin{equation}
% \ten{S} = {\mathbb{T}^{ - 1}}\left[\mathbb{F}\left( {{\Lambda _{{\lambda}}}\left( {\mathbb{T}{\mathbb{F}^{ - 1}}\left[ {\ten{M} - \frac{{\sum\nolimits_i {{\lambda_i}{\text{Fold}_i}\left( {{\mat{L}_i}} \right)} }}{{\sum\nolimits_i {{\lambda_i}} }}} \right]} \right)} \right)\right ].
% \end{equation}

% \item Sub-$\ten{M}$ problem: finally we fix $\{ \mat{L}_i\}$ and $\ten{S}$, and update $\ten{M}$ by solving
% \begin{equation}
% \label{eq:sub-M}
% \begin{aligned}
%  \mathop {\min }\limits_\ten{M} \quad & \sum\limits_{i = 1}^n {\frac{{{\lambda_i}}}{2}\left\| {{\mat{L}_i} + {\mat{S}_{(i)}} - {\mat{M}_{(i)}}} \right\|_F^2}\\
%   \st \quad & {\ten{M}_\Omega } = {\ten{T}_\Omega }. 
% \end{aligned}
% \end{equation}
% This sub-problem updates the reconstructed tensor and makes it consistent with the observed data. 
% The solution to Eq.~\reff{eq:sub-M} is given by
% \begin{equation}
% \small
%  {\ten{M}_{{i_1} \ldots {i_n}}} = \left\{ {
%  \begin{array}{cc}
% {{{\left( {\frac{{\sum\nolimits_i {{\lambda_i}{\text{Fold}_i}\left( {{\mat{L}_i}} \right)} }}{{\sum\nolimits_i {{\lambda_i}} }} + \ten{S}} \right)}_{{i_1}, \ldots ,{i_n}}}} & {\left( {{i_1}, \ldots ,{i_n}} \right) \notin \Omega }  \\
% {{\ten{T}_{{i_1}, \ldots ,{i_n}}}} & {\left( {{i_1}, \ldots ,{i_n}} \right) \in \Omega }
%  \end{array} } \right.   
% \end{equation}
% \end{itemize}





According to~\cite{tseng2001convergence}, the above implementation is guaranteed to converge to a coordinate-wise minimum point and stationary point since our function holds the separability and regularity properties. Different from~\cite{liu2012tensor}, our method cannot ensure global convergence since the additional $\ell_1$-norm term is not strictly convex \hzc{when the number of variables p $>$ the number of observations n}, thus the optimal solution may not be unique~\cite{tibshirani2013lasso}. 
However, the additional sparsity term does help for reconstruction, which will be shown in our experiments.
% Not compared with L Tensor structure 
\end{comment}
\begin{comment}
\subsection{Alternating Direction Method of Multipliers for Eq.~\reff{eq:raw_Obj}}
The alternating direction method of multipliers (ADMM) does not relax the equality constraint in Eq.~\reff{eq:raw_Obj}. Instead, it introduces some additional dual variables to handle the constraints.
In our tensor completion formulation, it is essentially a consensus ADMM approach~\cite{boyd2011distributed} to decompose the original problem.
The original problem in~\reff{eq:raw_Obj} is transformed to a problem of minimizing the augmented Lagrangian function: 
\begin{equation}\label{eq:admm_Obj}
\begin{aligned}
\mathop {\min } \quad& L_\rho(\ten{M},{\mat{L}_1},\ldots,{\mat{L}_n},\ten{S},{\ten{Y}_1},\ldots,{\ten{Y}_n})\\
\st \quad & {\ten{M}_\Omega } = {\ten{T}_\Omega },
\end{aligned}
\end{equation}
with
\begin{equation}
\begin{aligned}
 & L_\rho(\ten{M},{\mat{L}_1},\ldots,{\mat{L}_n},\ten{S},{\ten{Y}_1},\ldots,{\ten{Y}_n})\\
= & \sum\limits_{i = 1}^n \left[{{\alpha_i}{{\left\| {{\mat{L}_i}} \right\|}_ * }} + \frac{\rho}{2}\left\| {{\mat{L}_i} + {\mat{S}_{(i)}} - {\mat{M}_{(i)}}} \right\|_F^2 + \\
& \left \langle \ten{M} - \text{Fold}_i({\mat{L}_i}) - \ten{S}, {\ten{Y}_i} \right \rangle \right] + {\lambda}{\left\| \mathbb{T}{\mathbb{F}^{-1}}S \right\|_1}.
\end{aligned}
\end{equation}
Similarly, Eq.~\reff{eq:admm_Obj} can be also efficiently solved in an alternating scheme. In every iteration, the subproblems are shown in appendix~\ref{sec:appendix_admm} and the updating rules are listed as follows:
%minimize ${L_\rho}$ with only an observation consistent constraint (${\ten{M}_\Omega } = {\ten{T}_\Omega }$), which can also be solved alternatively. 
%that minimizing $L_\rho$ over variables ${\ten{M},\left\{\mat{L}_i\right\}^n_{i=1},\ten{S},\left\{\ten{Y}_i\right\}^n_{i=1},=}
% The dual variable $\ten{Y}_i$ is updated as:
% \begin{equation}\label{eq:admm_Y}
%     \ten{Y}_i= \ten{Y}_i-\rho({\text{Fold}_i}\left( {{\mat{L}_i}} \right)+\ten{S}-\ten{M}).
% \end{equation}
%The other variables are updated as the solutions to the corresponding sub-problems, which are shown in the appendix~\ref{sec:appendix_admm}. We list the update rule as follows:
\begin{equation}\label{eq:admm_L}
{\mat{L}_i} = {\text{SVT}_{\frac{{{\alpha_i}}}{{\rho}}}}\left( {{\mat{M}_{\left( i \right)}} -  {\mat{S}_{(i)}}} + \frac{1}{\rho} \mat{Y}_{i(i)} \right), \quad i=1,\ldots,n.
\end{equation}
\begin{equation}\label{eq:admm_S}
\ten{S} = {\mathbb{T}^{ - 1}}\left[\mathbb{F}\left( {{\Lambda _{\frac{\lambda}{\rho}}}\left( {\mathbb{T}{\mathbb{F}^{ - 1}}\left[ {\ten{M} -
{\sum\nolimits_i (\frac{{\mat{L}_i}}{n}}-\frac{\mat{Y}_{i(i)}}{n \rho})}\right]}\right)}\right)\right].
\end{equation}

\begin{equation}
    \label{eq:admm_M}
    \begin{array}{l}
    {m_{{i_1} \ldots {i_n}}} = 
    \left\{{ 
    \begin{array}{cc}
    {{{\hat{m}}_{{i_1}, \ldots ,{i_n}}}}, & \text{if } {\left( {{i_1}, \ldots ,{i_n}} \right) \notin \Omega }  \\
    {{t_{{i_1}, \ldots ,{i_n}}}}, & {\text{otherwise} }
    \end{array} } \right. \\
    \text{with tensor }   {\hat{\ten{M}}} =
    {
\sum_{i} ({{\text{Fold}_i}\left( {{\mat{L}_i}} \right)} 
+ \ten{S} - \frac{1}{\rho}{\ten{Y}_i}) / n}.
\end{array}
\end{equation}
    
%\begin{equation}\label{eq:admm_M}
% \begin{array}{l}
% {\ten{M}_{{i_1} \ldots {i_n}}} = \\
% \left\{ {
%  \begin{array}{cc}
% {{{\left( 
% {\frac{
% \sum\nolimits_i ({{\text{Fold}_i}\left( {{\mat{L}_i}} \right)} 
% + \ten{S} - \frac{1}{\rho}{\ten{Y}_i})}{n}}
% \right)}_{{i_1}, \ldots ,{i_n}}}} & {\left( {{i_1}, \ldots ,{i_n}} \right) \notin \Omega }  \\
% {{\ten{T}_{{i_1}, \ldots ,{i_n}}}} & {\left( {{i_1}, \ldots ,{i_n}} \right) \in \Omega. }
% \end{array} } \right.  
% \end{array}
% \end{equation}
\begin{equation}\label{eq:admm_Y}
    \ten{Y}_i= \ten{Y}_i-\rho({\text{Fold}_i}\left( {{\mat{L}_i}} \right)+\ten{S}-\ten{M}).
\end{equation}
\begin{algorithm}[t]
  \caption{Alternating solvers to Eq.~\reff{eq:raw_Obj}.}
  \label{alg:alt_solver}
  \KwIn{Initial $k$-space data $\ten{M}$ with ${\ten{M}_\Omega } = {\ten{T}_\Omega }$, maximum iteration $J$}
  %threshold parameter $\lambda_{Ei}$, mode weight $\lambda_{Li}$, sparsity regularization $\lambda_S$, and maximum iteration $K$}
  \KwOut{Reconstructed tensor $\ten{M}$, mode approximations ${\{\tilde{\ten{M}}_i}\}^n_{i=1}$}
  \For{$j =1,2,\dots,J$}
  { 
  \If{BCD}{
    \For{$i =1,2, \ldots ,n$}
        {
        update ${\mat{L}_i}$ via Eq.~\reff{eq:BCD_L}}\\
        
    
   Update $\ten{S}$ via Eq.~\reff{eq:BCD_S}%\quad \% Sub-$\ten{S}$\\
   
   Update ${\ten{M}}$ via Eq.~\reff{eq:BCD_M}%\quad \% Sub-$\ten{M}$ 
   }
   
   \If{ADMM}{
   \For{$i =1,2, \ldots ,n$}
    {Update ${\mat{L}_i}$ via Eq.~\reff{eq:admm_L}}
    
       Update $\ten{S}$ via Eq.~\reff{eq:admm_S}
   
   Update ${\ten{M}}$ via Eq.~\reff{eq:admm_M}
   
   \For{$i =1,2, \ldots ,n$}
        {
        Update ${\ten{Y}_i}$ via Eq.~\reff{eq:admm_Y}\\
        }
  } 
  }
  Calculate ${\{\tilde{\ten{M}}_i}\}^n_{i=1}$ via Eq.~\reff{eq:mode_appro} %\quad \%mode information
\end{algorithm}

The complete algorithm flow of solving the L+S tensor completion problem, which includes both block coordinate descent and ADMM, is summarized in Algorithm~\ref{alg:alt_solver}.


The ADMM solver also converges to a coordinate-wise minimum since it follows the same decomposition scheme with an additional dual variable. The main advantage of ADMM is dealing with the inequality constraints directly and having a more accurate formulation. The convergence rate of ADMM is still under investigation, but the experiments show that ADMM usually performs outperforms block coordinate descent in the practice, which will be shown later.

It is worth emphasizing that the constructed modes are not equivalent to each other although the inequalities of Eq.~\reff{eq:raw_Obj} are not relaxed. 
The tensor nuclear norm included in the objective function leads to different objectives in the decomposed $\{\text{Sub-}{\mat{L}_i}\}_{i=1}^n$ problems (see appendix~\ref{sec:appendix_admm}), therefore different solutions will be obtained for different modes. 
In the next section, we will show that this difference is the key to design our active sampling method.

% To make the completion model converges faster, one trick is to update the mode weights ${\lambda_{Li}}$ adaptively. 
% %This setting also reduces the burden of tuning weight parameters. %
% After one iteration of $\ten{S}$ and all ${\mat{L}_i}$ blocks, we can calculate the tr 
% The tensor completion algorithm is summarized in Alg.~\ref{alg:TC_framework}. Besides the reconstructed tensor $\ten{M}$, we also obtain approximations to all modes ${\{\tilde{\ten{M}}_i}\}^n_{i=1}$, which will be introduced in the next subsection.
%In the implementation, error regularization $\lambda_{Ei}$ can be fixed as constants, and we only need to tune $\lambda_{Li}$ and $\lambda_S$. Weight adaption. 
%\floatname{algorithm}{Alg.}


% \begin{algorithm}[t]
%   \caption{ADMM solver to Eq.~\reff{eq:raw_Obj}.}
%   \label{alg:admm}
%   \KwIn{Initial $\ten{M}$ with ${\ten{M}_\Omega } = {\ten{T}_\Omega }$, positive parameter $\rho$, mode weight $\lambda_{Li}$, sparsity regularization $\lambda_S$ and maximum iteration $K$}
%   \KwOut{Reconstructed tensor $\ten{M}$, mode approximations ${\{\tilde{\ten{M}}_i}\}^n_{i=1}$}
%   \For{$k =1,2,\dots,K$}
%   { 
%     \For{$i =1,2, \ldots ,n$}
%         {
%         Update ${\mat{L}_i}$ via Eq.~\reff{eq:admm_L}
%         }

%   Update $\ten{S}$ via Eq.~\reff{eq:admm_S}
   
%   Update ${\ten{M}}$ via Eq.~\reff{eq:admm_M}
   
%   \For{$i =1,2, \ldots ,n$}
%         {
%         Update ${\ten{Y}_i}$ via Eq.~\reff{eq:admm_Y}\\
%         }
%   } 
%   Calculate ${\{\tilde{\ten{M}}_i}\}^n_{i=1}$ via Eq.~\reff{eq:mode_appro} %\quad \%mode information
% \end{algorithm}



% Possible ways to make the formulation complete/better:
% 1. Sparsity transformation
% 2. L\&S structure
% 3. Lagranian augmented: ROBUST LOW-RANK TENSOR RECOVERY: MODELS AND ALGORITHMS
\end{comment}







==> related_works.tex <==
\section{Related works}
\label{sec:related_works}
\par
\textbf{Tensor Methods for MRI Reconstruction:}
Tensor has been employed in the MR imaging since the ambient dimension of MRI data sets is often high. 
%lots of MRI data naturally hold a high-dimensional structure.
Yang~\etal~\cite{yang2017dynamic} showed that low-rank tensor completion with a sparsity regularizer could accelerate MRI reconstruction.
%\cite{banco2016sampling} summarized several tensor models for MRI data.
Christodoulou~\etal~\cite{christodoulou2018magnetic} applied low-rank tensor modeling for motion-resolved quantitative imaging.
The sparse transform of compressive-sensing MRI is formulated as a Tucker tensor decomposition in~\cite{yu2014multidimensional}. 
Liu~\etal~\cite{liu2018accelerated} proposed a phase-constrained low-rank model for high b-value diffusion-weighted MRI.
The theory of regular sub-Nyquist samplings for tensor completion was studied in \cite{kanatsoulis2019tensor}.
He~\etal~\cite{he2016accelerated} firstly estimated an explicit low-rank tensor subspace and reconstructed high-dimensional data via fitting the subspace. 
A locally low-rank tensor method for dynamic cardiac MRI reconstruction is proposed by Liu~\etal~\cite{liu2019dynamic}, where patch-based local structure is exploited. 
%Roohi~\etal~\cite{roohi2017multi} adopted a low-rank plus sparsity tensor structure for MRI reconstruction, but with a different optimization formulation.
Although tensor models have been exploited to enable MRI reconstruction from highly-undersampled data, this paper is the first to leverage tensor model for active sampling in MR imaging. 
%Although various tensor models have been reported for MRI reconstruction, to the best of our knowledge this paper is the first to consider adaptive sampling for tensor MRI data. 

\textbf{Experimental Design for MRI:} 
Experimental design or active sampling is an important approach to accelerate MRI reconstruction.
Seeger~\etal~\cite{seeger2010optimization} proposed a Bayesian experimental design framework by maximizing the information gain.
A learning-based method was proposed in \cite{gozcu2018learning} to select samples for compressive MRI.
Ravishankar~\etal~\cite{ravishankar2011adaptive} partitioned the sampling space and proposed an adaptive sampling pattern by moving the samples among blocks.
Zhao~\etal~\cite{zhao2018optimal} proposed an optimal experimental design to maximize the signal-to-noise ratio efficiency with estimation-theoretic bounds.
A self-supervised framework is proposed by Jin~\etal~\cite{jin2019self} to accelerate compressive MRI by considering both the data acquisition and the reconstruction process within a single deep network.
Zhang~\etal~\cite{zhang2019reducing} proposed an active acquisition model based on uncertainty reduction via introducing an evaluator network which evaluates the quality gain in reconstruction of each $k$-space measurement.

Once the MRI reconstruction is formulated as a matrix/ tensor completion problem, the experimental design becomes an active matrix/tensor completion problem. 
%Chouvardas~\etal~\cite{chouvardas2016method} adopts QBC strategy to identify informative areas of a map matrix. 
%\cite{ruchansky2015matrix} offers an active sampling according to the matrix structure from the perspective of a linear equation system.
Some researchers developed Bayesian frameworks for active matrix completion~\cite{chakraborty2013active,sutherland2013active}. 
Claude~\etal~\cite{claude2017efficient} offered an adaptive sampling method under smoothness assumption on matrix components. 
An entropy-driven approach for active matrix completion with uncertainty quantification was also proposed in~\cite{mak2017active}.

However, the active sampling for tensor completion problems is much less studied.
An adaptive tubal-sampling method is proposed for a 3D low-tubal-rank tensor completion~\cite{liu2015adaptive}, but it could not be generalized to higher-order tensors.
Krishnamurthy and Singh~\cite{krishnamurthy2013low} proposed a probabilistic sampling method to adaptively estimate and update the tensor singular subspace based on an incoherent condition. Both of them did not consider the pattern constraints in MRI sampling.
%and assumed an initialization of uniform sampling, which is infeasible in most MR images.
To the best of our knowledge, this work is the first to propose a deterministic active sampling method %for tensor MRI reconstruction with consideration of the pattern constraints in MRI measurement.
for tensor MR imaging while incorporating sampling constraint inherent in MR data acquisition process. 

%Compressive sensing MRI based on Leverage score~\cite{krahmer2013stable}.
% \par
% \textbf{Active matrix/tensor completion} Active matrix completion has been recently paid more attention by researchers.


%\textbf{L+S for MRI reconstruction:}
%Although L+S has been a classical structure in the image reconstruction field, our completion formulation is still valuable.  
% Our model extends the L+S MRI reconstruction framework~\cite{otazo2015low} to a high-dimensional $k$-space tensor case, where our target objection is direct $k$-space data. 
% Besides the MRI applications, the L+S structure is also widely used.
% Go decomposition~\cite{zhou2011godec} sets a prior setting on the matrix rank and sparsity level as the problem constraints, which is however not easy to know in the practice. 
% Robust PCA~\cite{candes2011robust} proposed an exact L+S decomposition to a matrix, but which may be not available under noise. 
% \cite{lu2016tensor} proposed a tensor robust PCA based on a special t-SVD nuclear norm, which is restricted for 3D tensor data.
% Some other papers used ADMM algorithm to solve the tensor L+S structure formulation~\cite{goldfarb2014robust,roohi2017multi}. 




==> tensor_completion.tex <==
\section{Low-rank Tensor-Format MRI Reconstruction}
\label{sec:ten_completion}
As shown in~\reff{eq:ten_nuclear}, $n$ mode matricization $\{{\mat{X}_{(i)}}\}^n_{i=1}$ represents the same set of data and thus are coupled to each other, which makes it hard to solve.
Therefore, we replace them with $n$ additional matrices $\{{\mat{X}_i}\}^n_{i=1}$ and introduce an additional tensor $\ten{M}$. The optimization problem can be reformulated as:
\begin{equation}\label{eq:raw_Obj}
\begin{aligned}
\mathop {\min }\limits_{\left\{\mat{X}_i\right\}^n_{i=1},\ten{M}} \quad & \sum\limits_{i = 1}^n {{\alpha_i}{{\left\| {{\mat{X}_i}} \right\|}_ * }}\\
\st \quad & {\mat{X}_ i} = {\mat{M}_{(i)}},\quad i = 1,2,\ldots,n\\
&{\ten{M}_\Omega } = {\ten{T}_\Omega }.
\end{aligned}
\end{equation}
where $\ten{M}$ is a tensor in the $k$-space; $\mat{M}_{(i)}$ is the $i$-th mode matricization of $\ten{M}$; $\ten{T}$ is the fully sampled $k$-space tensor and $\Omega$ is its observation set;
Essentially, we can model the low-rankness of both the $k$-space and image space data. 
We choose the former one since it enables the design of our active sampling methods in Section~\ref{sec:active_strategy}.
If the MRI data is known to hold some additional structure, we can further modify the imagining model by adding a regularization term, like the low rank plus sparsity model~\cite{roohi2017multi}.

Eq.~\reff{eq:raw_Obj} can be efficiently solved via some alternating solvers, like block coordinate descent and alternating direction method of multipliers (ADMM)~\cite{liu2012tensor}. 
Our proposed active sampling strategies will exploit these additional mode approximations $\left\{\mat{X}_i\right\}^n_{i=1}$ to acquire new $k$-space samples.
The complete flowchart of our MRI reconstruction framework is illustrated in Fig.~\ref{fig:whole_framework}.
\begin{figure}[!t]
    \centering
    \includegraphics[scale=0.4]{Figure/framework.png}
    \caption{Flowchart of the MRI reconstruction framework.}
    \label{fig:whole_framework}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{comment}
\subsection{Block Coordinate Descent Solver to Eq.~\reff{eq:raw_Obj}} 
The first equality constraint in Eq.~\reff{eq:raw_Obj} still makes the variables coupled to each other. To address this issue, we further relax the problem and convert it to the following one:
%To address this issue, we further relax it as:
% \begin{equation}
% {\left\| {{\mat{M}_{\left( i \right)}} - {\mat{L}_i} - {\mat{S}_{\left( i \right)}}} \right\|_F} \le {\epsilon_i}, \quad i = 1,2,\ldots,n,   
% \end{equation}
%where %${\left\|  \cdot  \right\|_F}$ is the matrix Frobenius norm and 
%${\epsilon_i}$ is a numerical threshold for approximation.
%Then the problem can be converted into the following equivalent one: 
\begin{equation} \label{eq:BCD_Obj}
\begin{aligned}
\min_\limits_{\left\{\mat{L}_i\right\}^n_{i=1},\ten{S},\ten{M}} \quad & 
\sum\limits_{i = 1}^n ({{\alpha_i}{{\left\| {\mat{L}_i} \right\|}_ * }}  + \frac{{\lambda_i}}{{2}}\left\| {{\ten{L}_ i} + {\mat{S}_{(i)}} - {\mat{M}_{(i)}}} \right\|_F^2) \\
& + {\lambda}{\left\| \mathbb{T}{\mathbb{F}^{-1}}\ten{S} \right\|_1}\\
\st \quad  &{\ten{M}_\Omega } = {\ten{T}_\Omega }
\end{aligned}
\end{equation}
where $\lambda_i$ is a fixed positive constant associated with each relaxed constraint. The resulting problem~\eqref{eq:BCD_Obj} is convex and decoupled, and it can be easily solved via a block coordinate descent (BCD) algorithm. 

The block coordinate descent method divides all variables into several groups and solves a sub-problem of each group while keeping others fixed. 
Specifically, we divide all variables into $n+2$ groups: $\left\{ {{\mat{L}_i}} \right\}_{i = 1}^n$, $\ten{S}$, and $\ten{M}$. 
%Then each group of variables can be updated with a closed-form solution during the iteration. 
In every iteration, the subproblems shown in appendix~\ref{sec:appendix_BCD} are solved with the following closed-form updates: 
\begin{itemize}[leftmargin=*]

    \item Update ${\mat{L}_i}$: 
    \begin{equation}\label{eq:BCD_L}
    {\mat{L}_i} = {\text{SVT}_{\frac{{{\alpha_i}}}{{{\lambda _i}}}}}\left( {{\mat{M}_{\left( i \right)}} -  {\mat{S}_{(i)}}} \right).
    \end{equation}
    Here $\text{SVT}(\cdot)$ denotes a singular value thresholding operator~\cite{cai2010singular}. Let $\mat{X} = \mat{U}\mat{{\Sigma }}\mat{{V^H}}$ be a singular value decomposition, then ${\text{SVT}_\tau }\left( \mat{X} \right) = \mat{U}\mat{{\Sigma _\tau }}\mat{{V^H}}$. Here $\mat{\Sigma}_\tau$ is a diagonal matrix and its $i$-th element is $ \max (\sigma_i - \tau, 0)$ with $\sigma_i$ being the $i$-th largest singular value of $\mat{X}$. 
    \item Update $\ten{S}$:
    \begin{equation}\label{eq:BCD_S}
    \ten{S} = {\mathbb{T}^{ - 1}}\left[\mathbb{F}\left( {{\Lambda _{{\lambda}}}\left( {\mathbb{T}{\mathbb{F}^{ - 1}}\left[ {\ten{M} - \frac{{\sum\nolimits_i {{\lambda_i}{\text{Fold}_i}\left( {{\mat{L}_i}} \right)} }}{{\sum\nolimits_i {{\lambda_i}} }}} \right]} \right)} \right)\right ].
    \end{equation}
    Here ${\Lambda _\lambda }\left( x \right)$ denotes a soft-thresholding operator ${\Lambda _\lambda }\left( x \right) = \frac{x}{{\left| x \right|}}\max \left( {\left| x \right| - \lambda ,0} \right)$
    where $\left|x\right|$ is the amplitude of a complex number $x$. The operator $\Lambda(\cdot)$ can be extended to a matrix or tensor case by applying it on each element. 
    
    \item Update $\ten{M}$: each element is updated as follows:
    \begin{equation}
    \label{eq:BCD_M}
    \begin{array}{l}
    {m_{{i_1} \ldots {i_n}}} = 
    \left\{{ 
    \begin{array}{cc}
    {{{\hat{m}}_{{i_1}, \ldots ,{i_n}}}}, & \text{if } {\left( {{i_1}, \ldots ,{i_n}} \right) \notin \Omega }  \\
    {{t_{{i_1}, \ldots ,{i_n}}}}, & {\text{otherwise} }
    \end{array} } \right. \\
    \text{with tensor }   {\hat{\ten{M}}} ={ {\frac{{\sum\nolimits_i {{\lambda_i}{\text{Fold}_i}\left( {{\mat{L}_i}} \right)} }}{{\sum\nolimits_i {{\lambda_i}} }} + \ten{S}. }} 
 \end{array}
    \end{equation}
    Here $t_{i_1 i_2 \cdots i_n}$ denotes one element of $\ten{T}$.
\end{itemize}



% Every iteration of the BCD solves the following sub-problems: 
% %\zz{You didn't fix my comments in the email.}
% \begin{itemize}

%     \item Sub-${\mat{L}_i}$ problem: fixing $\ten{S}$ and $\ten{M}$, we update $\{ \mat{L}_i\}$ by solving the following problem:
% \begin{equation}
% \label{eq:sub-L}
% \begin{array}{ll}
% \mathop {\min } \limits_{\{\mat{L}_i\}} & \sum\limits_{i = 1}^n {{\alpha_i}{{\left\| {{\mat{L}_i}} \right\|}_*}}  + \frac{{{\lambda_i}}}{2}\left\| {{\mat{L}_i} + {\mat{S}_{(i)}} - {\mat{M}_{(i)}}} \right\|_F^2 \\
% & \equiv \sum\limits_{i = 1}^n \frac{1}{2}\left\| {{\mat{L}_i} + {\mat{S}_{(i)}} - {\mat{M}_{(i)}}} \right\|_F^2 + \frac{{{\alpha_i}}}{{{\lambda_i}}}{\left\| {{\mat{L}_i}} \right\|_*}.
% \end{array}
% \end{equation} 
% To solve Eq.~\reff{eq:sub-L}, we need to use a singular value thresholding (SVT) operator~\cite{cai2010singular}.
% Let $\mat{X} = \mat{U}\mat{{\Sigma }}\mat{{V^H}}$ be the singular value decomposition for $X$. Then the singular value thresholding operator ${\text{SVT}_\lambda }\left( \mat{X} \right)$ is defined as ${\text{SVT}_\lambda }\left( \mat{X} \right) = \mat{U}\mat{{\Sigma _\lambda }}\mat{{V^H}}$, where $\mat{\Sigma _\lambda} = \text{diag}(\max (\sigma_i - \lambda, 0))$ and $\sigma_i$ is the $i$th largest singular value. 
% Note that here the matrix $\mat{X}$ is complex, thus the conjugate transpose is used. 
% We can easily compute the optimal ${\mat{L}_i}$ as:
% \begin{equation}
% {\mat{L}_i} = {\text{SVT}_{\frac{{{\alpha_i}}}{{{\lambda _e}}}}}\left( {{\mat{M}_{\left( i \right)}} -  {\mat{S}_{(i)}}} \right).
% \end{equation}

% \item Sub-$\ten{S}$ problem: we fix $\{ \mat{L}_i\}$ and $\ten{M}$, then update $\ten{S}$ by solving
% \begin{equation}
% \label{eq:sub-S}
% \begin{array}{ll}
% \mathop {\min }\limits_{\ten{S}} & \sum\limits_{i = 1}^n \frac{{{\lambda_i}}}{2}\left\| {{\mat{L}_i} + {\mat{S}_{(i)}} - {\mat{M}_{(i)}}} \right\|_F^2 + {\lambda}{\left\| {\mathbb{T}{\mathbb{F}^{-1}}\ten{S}} \right\|_1}\\
% \end{array}
% \end{equation}
% To solve Eq.~\reff{eq:sub-S}, a soft-thresholding operator 
% ${\Lambda _\lambda }\left( x \right) = \frac{x}{{\left| x \right|}}\max \left( {\left| x \right| - \lambda ,0} \right)$ 
% is defined, where $\left|x\right|$ is the amplitude of a complex number $x$. 
% %\zz{(Please consider using another notation for the soft thresholding operator, because it's very similar to the aquisition operator in Eq. (4).) }
% The operator $\Lambda$ can be generalized to a tensor case when we apply it to each entry.
% The solution of Eq.~\reff{eq:sub-S} is given by
% \begin{equation}
% \ten{S} = {\mathbb{T}^{ - 1}}\left[\mathbb{F}\left( {{\Lambda _{{\lambda}}}\left( {\mathbb{T}{\mathbb{F}^{ - 1}}\left[ {\ten{M} - \frac{{\sum\nolimits_i {{\lambda_i}{\text{Fold}_i}\left( {{\mat{L}_i}} \right)} }}{{\sum\nolimits_i {{\lambda_i}} }}} \right]} \right)} \right)\right ].
% \end{equation}

% \item Sub-$\ten{M}$ problem: finally we fix $\{ \mat{L}_i\}$ and $\ten{S}$, and update $\ten{M}$ by solving
% \begin{equation}
% \label{eq:sub-M}
% \begin{aligned}
%  \mathop {\min }\limits_\ten{M} \quad & \sum\limits_{i = 1}^n {\frac{{{\lambda_i}}}{2}\left\| {{\mat{L}_i} + {\mat{S}_{(i)}} - {\mat{M}_{(i)}}} \right\|_F^2}\\
%   \st \quad & {\ten{M}_\Omega } = {\ten{T}_\Omega }. 
% \end{aligned}
% \end{equation}
% This sub-problem updates the reconstructed tensor and makes it consistent with the observed data. 
% The solution to Eq.~\reff{eq:sub-M} is given by
% \begin{equation}
% \small
%  {\ten{M}_{{i_1} \ldots {i_n}}} = \left\{ {
%  \begin{array}{cc}
% {{{\left( {\frac{{\sum\nolimits_i {{\lambda_i}{\text{Fold}_i}\left( {{\mat{L}_i}} \right)} }}{{\sum\nolimits_i {{\lambda_i}} }} + \ten{S}} \right)}_{{i_1}, \ldots ,{i_n}}}} & {\left( {{i_1}, \ldots ,{i_n}} \right) \notin \Omega }  \\
% {{\ten{T}_{{i_1}, \ldots ,{i_n}}}} & {\left( {{i_1}, \ldots ,{i_n}} \right) \in \Omega }
%  \end{array} } \right.   
% \end{equation}
% \end{itemize}





According to~\cite{tseng2001convergence}, the above implementation is guaranteed to converge to a coordinate-wise minimum point and stationary point since our function holds the separability and regularity properties. Different from~\cite{liu2012tensor}, our method cannot ensure global convergence since the additional $\ell_1$-norm term is not strictly convex \hzc{when the number of variables p $>$ the number of observations n}, thus the optimal solution may not be unique~\cite{tibshirani2013lasso}. 
However, the additional sparsity term does help for reconstruction, which will be shown in our experiments.
% Not compared with L Tensor structure 
\end{comment}
\begin{comment}
\subsection{Alternating Direction Method of Multipliers for Eq.~\reff{eq:raw_Obj}}
The alternating direction method of multipliers (ADMM) does not relax the equality constraint in Eq.~\reff{eq:raw_Obj}. Instead, it introduces some additional dual variables to handle the constraints.
In our tensor completion formulation, it is essentially a consensus ADMM approach~\cite{boyd2011distributed} to decompose the original problem.
The original problem in~\reff{eq:raw_Obj} is transformed to a problem of minimizing the augmented Lagrangian function: 
\begin{equation}\label{eq:admm_Obj}
\begin{aligned}
\mathop {\min } \quad& L_\rho(\ten{M},{\mat{L}_1},\ldots,{\mat{L}_n},\ten{S},{\ten{Y}_1},\ldots,{\ten{Y}_n})\\
\st \quad & {\ten{M}_\Omega } = {\ten{T}_\Omega },
\end{aligned}
\end{equation}
with
\begin{equation}
\begin{aligned}
 & L_\rho(\ten{M},{\mat{L}_1},\ldots,{\mat{L}_n},\ten{S},{\ten{Y}_1},\ldots,{\ten{Y}_n})\\
= & \sum\limits_{i = 1}^n \left[{{\alpha_i}{{\left\| {{\mat{L}_i}} \right\|}_ * }} + \frac{\rho}{2}\left\| {{\mat{L}_i} + {\mat{S}_{(i)}} - {\mat{M}_{(i)}}} \right\|_F^2 + \\
& \left \langle \ten{M} - \text{Fold}_i({\mat{L}_i}) - \ten{S}, {\ten{Y}_i} \right \rangle \right] + {\lambda}{\left\| \mathbb{T}{\mathbb{F}^{-1}}S \right\|_1}.
\end{aligned}
\end{equation}
Similarly, Eq.~\reff{eq:admm_Obj} can be also efficiently solved in an alternating scheme. In every iteration, the subproblems are shown in appendix~\ref{sec:appendix_admm} and the updating rules are listed as follows:
%minimize ${L_\rho}$ with only an observation consistent constraint (${\ten{M}_\Omega } = {\ten{T}_\Omega }$), which can also be solved alternatively. 
%that minimizing $L_\rho$ over variables ${\ten{M},\left\{\mat{L}_i\right\}^n_{i=1},\ten{S},\left\{\ten{Y}_i\right\}^n_{i=1},=}
% The dual variable $\ten{Y}_i$ is updated as:
% \begin{equation}\label{eq:admm_Y}
%     \ten{Y}_i= \ten{Y}_i-\rho({\text{Fold}_i}\left( {{\mat{L}_i}} \right)+\ten{S}-\ten{M}).
% \end{equation}
%The other variables are updated as the solutions to the corresponding sub-problems, which are shown in the appendix~\ref{sec:appendix_admm}. We list the update rule as follows:
\begin{equation}\label{eq:admm_L}
{\mat{L}_i} = {\text{SVT}_{\frac{{{\alpha_i}}}{{\rho}}}}\left( {{\mat{M}_{\left( i \right)}} -  {\mat{S}_{(i)}}} + \frac{1}{\rho} \mat{Y}_{i(i)} \right), \quad i=1,\ldots,n.
\end{equation}
\begin{equation}\label{eq:admm_S}
\ten{S} = {\mathbb{T}^{ - 1}}\left[\mathbb{F}\left( {{\Lambda _{\frac{\lambda}{\rho}}}\left( {\mathbb{T}{\mathbb{F}^{ - 1}}\left[ {\ten{M} -
{\sum\nolimits_i (\frac{{\mat{L}_i}}{n}}-\frac{\mat{Y}_{i(i)}}{n \rho})}\right]}\right)}\right)\right].
\end{equation}

\begin{equation}
    \label{eq:admm_M}
    \begin{array}{l}
    {m_{{i_1} \ldots {i_n}}} = 
    \left\{{ 
    \begin{array}{cc}
    {{{\hat{m}}_{{i_1}, \ldots ,{i_n}}}}, & \text{if } {\left( {{i_1}, \ldots ,{i_n}} \right) \notin \Omega }  \\
    {{t_{{i_1}, \ldots ,{i_n}}}}, & {\text{otherwise} }
    \end{array} } \right. \\
    \text{with tensor }   {\hat{\ten{M}}} =
    {
\sum_{i} ({{\text{Fold}_i}\left( {{\mat{L}_i}} \right)} 
+ \ten{S} - \frac{1}{\rho}{\ten{Y}_i}) / n}.
\end{array}
\end{equation}
    
%\begin{equation}\label{eq:admm_M}
% \begin{array}{l}
% {\ten{M}_{{i_1} \ldots {i_n}}} = \\
% \left\{ {
%  \begin{array}{cc}
% {{{\left( 
% {\frac{
% \sum\nolimits_i ({{\text{Fold}_i}\left( {{\mat{L}_i}} \right)} 
% + \ten{S} - \frac{1}{\rho}{\ten{Y}_i})}{n}}
% \right)}_{{i_1}, \ldots ,{i_n}}}} & {\left( {{i_1}, \ldots ,{i_n}} \right) \notin \Omega }  \\
% {{\ten{T}_{{i_1}, \ldots ,{i_n}}}} & {\left( {{i_1}, \ldots ,{i_n}} \right) \in \Omega. }
% \end{array} } \right.  
% \end{array}
% \end{equation}
\begin{equation}\label{eq:admm_Y}
    \ten{Y}_i= \ten{Y}_i-\rho({\text{Fold}_i}\left( {{\mat{L}_i}} \right)+\ten{S}-\ten{M}).
\end{equation}
\begin{algorithm}[t]
  \caption{Alternating solvers to Eq.~\reff{eq:raw_Obj}.}
  \label{alg:alt_solver}
  \KwIn{Initial $k$-space data $\ten{M}$ with ${\ten{M}_\Omega } = {\ten{T}_\Omega }$, maximum iteration $J$}
  %threshold parameter $\lambda_{Ei}$, mode weight $\lambda_{Li}$, sparsity regularization $\lambda_S$, and maximum iteration $K$}
  \KwOut{Reconstructed tensor $\ten{M}$, mode approximations ${\{\tilde{\ten{M}}_i}\}^n_{i=1}$}
  \For{$j =1,2,\dots,J$}
  { 
  \If{BCD}{
    \For{$i =1,2, \ldots ,n$}
        {
        update ${\mat{L}_i}$ via Eq.~\reff{eq:BCD_L}}\\
        
    
   Update $\ten{S}$ via Eq.~\reff{eq:BCD_S}%\quad \% Sub-$\ten{S}$\\
   
   Update ${\ten{M}}$ via Eq.~\reff{eq:BCD_M}%\quad \% Sub-$\ten{M}$ 
   }
   
   \If{ADMM}{
   \For{$i =1,2, \ldots ,n$}
    {Update ${\mat{L}_i}$ via Eq.~\reff{eq:admm_L}}
    
       Update $\ten{S}$ via Eq.~\reff{eq:admm_S}
   
   Update ${\ten{M}}$ via Eq.~\reff{eq:admm_M}
   
   \For{$i =1,2, \ldots ,n$}
        {
        Update ${\ten{Y}_i}$ via Eq.~\reff{eq:admm_Y}\\
        }
  } 
  }
  Calculate ${\{\tilde{\ten{M}}_i}\}^n_{i=1}$ via Eq.~\reff{eq:mode_appro} %\quad \%mode information
\end{algorithm}

The complete algorithm flow of solving the L+S tensor completion problem, which includes both block coordinate descent and ADMM, is summarized in Algorithm~\ref{alg:alt_solver}.


The ADMM solver also converges to a coordinate-wise minimum since it follows the same decomposition scheme with an additional dual variable. The main advantage of ADMM is dealing with the inequality constraints directly and having a more accurate formulation. The convergence rate of ADMM is still under investigation, but the experiments show that ADMM usually performs outperforms block coordinate descent in the practice, which will be shown later.

It is worth emphasizing that the constructed modes are not equivalent to each other although the inequalities of Eq.~\reff{eq:raw_Obj} are not relaxed. 
The tensor nuclear norm included in the objective function leads to different objectives in the decomposed $\{\text{Sub-}{\mat{L}_i}\}_{i=1}^n$ problems (see appendix~\ref{sec:appendix_admm}), therefore different solutions will be obtained for different modes. 
In the next section, we will show that this difference is the key to design our active sampling method.

% To make the completion model converges faster, one trick is to update the mode weights ${\lambda_{Li}}$ adaptively. 
% %This setting also reduces the burden of tuning weight parameters. %
% After one iteration of $\ten{S}$ and all ${\mat{L}_i}$ blocks, we can calculate the tr 
% The tensor completion algorithm is summarized in Alg.~\ref{alg:TC_framework}. Besides the reconstructed tensor $\ten{M}$, we also obtain approximations to all modes ${\{\tilde{\ten{M}}_i}\}^n_{i=1}$, which will be introduced in the next subsection.
%In the implementation, error regularization $\lambda_{Ei}$ can be fixed as constants, and we only need to tune $\lambda_{Li}$ and $\lambda_S$. Weight adaption. 
%\floatname{algorithm}{Alg.}


% \begin{algorithm}[t]
%   \caption{ADMM solver to Eq.~\reff{eq:raw_Obj}.}
%   \label{alg:admm}
%   \KwIn{Initial $\ten{M}$ with ${\ten{M}_\Omega } = {\ten{T}_\Omega }$, positive parameter $\rho$, mode weight $\lambda_{Li}$, sparsity regularization $\lambda_S$ and maximum iteration $K$}
%   \KwOut{Reconstructed tensor $\ten{M}$, mode approximations ${\{\tilde{\ten{M}}_i}\}^n_{i=1}$}
%   \For{$k =1,2,\dots,K$}
%   { 
%     \For{$i =1,2, \ldots ,n$}
%         {
%         Update ${\mat{L}_i}$ via Eq.~\reff{eq:admm_L}
%         }

%   Update $\ten{S}$ via Eq.~\reff{eq:admm_S}
   
%   Update ${\ten{M}}$ via Eq.~\reff{eq:admm_M}
   
%   \For{$i =1,2, \ldots ,n$}
%         {
%         Update ${\ten{Y}_i}$ via Eq.~\reff{eq:admm_Y}\\
%         }
%   } 
%   Calculate ${\{\tilde{\ten{M}}_i}\}^n_{i=1}$ via Eq.~\reff{eq:mode_appro} %\quad \%mode information
% \end{algorithm}



% Possible ways to make the formulation complete/better:
% 1. Sparsity transformation
% 2. L\&S structure
% 3. Lagranian augmented: ROBUST LOW-RANK TENSOR RECOVERY: MODELS AND ALGORITHMS
\end{comment}






